Computing Euclidean k-Center over Sliding Windows

In the Euclidean $k$-center problem in sliding window model, input points are given in a data stream and the goal is to find the $k$ smallest congruent balls whose union covers the $N$ most recent points of the stream. In this model, input points are allowed to be examined only once and the amount of space that can be used to store relative information is limited. Cohen-Addad et al.~\cite{cohen-2016} gave a $(6+\epsilon)$-approximation for the metric $k$-center problem using O($k/\epsilon \log \alpha$) points, where $\alpha$ is the ratio of the largest and smallest distance and is assumed to be known in advance. In this paper, we present a $(3+\epsilon)$-approximation algorithm for the Euclidean $1$-center problem using O($1/\epsilon \log \alpha$) points. We present an algorithm for the Euclidean $k$-center problem that maintains a coreset of size $O(k)$. Our algorithm gives a $(c+2\sqrt{3} + \epsilon)$-approximation for the Euclidean $k$-center problem using O($k/\epsilon \log \alpha$) points by using any given $c$-approximation for the coreset where $c$ is a positive real number. For example, by using the $2$-approximation~\cite{feder-greene-1988} of the coreset, our algorithm gives a $(2+2\sqrt{3} + \epsilon)$-approximation ($\approx 5.465$) using $O(k\log k)$ time. This is an improvement over the approximation factor of $(6+\epsilon)$ by Cohen-Addad et al.~\cite{cohen-2016} with the same space complexity and smaller update time per point. Moreover we remove the assumption that $\alpha$ is known in advance. Our idea can be adapted to the metric diameter problem and the metric $k$-center problem to remove the assumption. For low dimensional Euclidean space, we give an approximation algorithm that guarantees an even better approximation.

==> CHANGELOG <==
LIPICS Style - CHANGELOG

* 10/12/2018 LIPIcs-v2019 v2.0
** New Features
*** support of metadata in PDF file (e.g. author, title, keywords) 
*** revised displaying of author-related funding acknowledgements (now displayed as part of the funding block instead of footnotes)
*** added support for cleveref package (new document option 'cleveref')
*** added support for using autoref for theorem-like environments (new document option 'autoref')
*** added new environment claim and claimproof to realize sub-proofs
*** added new environment proposition
** Bugfixes
*** fixed problems with theorem-like environments when using cleveref and autoref (see new features above)
*** switched several URL from http to https
*** fixed problems with using of ACM 2012 classification (deactivated subjclass and revised support of ccsdesc macro)
** Minor changes
*** moved ORCID symbol behind author name (according https://orcid.org/content/journal-display-guidelines)
*** added separator \and to split several affiliations
*** added warnings when package 'enumitem' or 'paralist' are loaded; they manipulate the pre-defined enumeration styles and are partly incompatible
*** preloaded package 'microtype' in style
*** revised spacings/font sizes for top matter

* 09/04/2018 LIPIcs-v2018 v1.5
** Bugfixes
*** Fixed problem with page style in case of many authors
*** Fixed aggregation of authors for ToC file

* 15/03/2018 LIPIcs-v2018 v1.4
** Bugfixes
*** Fixed enumerations
*** Fixed aggregation of authors for ToC file

* 26/02/2018 LIPIcs-v2018 v1.3
** Bugfixes
*** Fixed \hideLIPIcs
*** Fixed enumerations
*** Fixed typo
** Revised display of ORCIDs following recommendation by ORCID

* 06/02/2018 LIPIcs-v2018 v1.2
** Release of LIPIcs-v2018
*** revised author macro \author{name}{affil}{email}{orcid}{funding} 
*** added support for ORCIDs
*** switched to ACM 2012 classification system
*** added new macros for extended metadata \category, \relatedversion, \supplement, \funding, \acknowledgements
*** added warnings for missing mandatory metadata
*** added preconfigured enumeration styles based on the enumerate package
*** added option \hideLIPIcs to hide all LIPIcs related information
*** added support for line numbers
** Bugfixes
*** fixed copyright line
*** added warning when using outdated subfig package due to incompatibilities in preloaded subcaption package
*** fixed bug when using MnSymbol package
*** fixed bug in numbering in theorem-like environments used in appendix
*** fixed problems in ToC file


==> includes/1-center.tex <==
\section{The 1-Center Problem}
\label{section:1-center}


\begin{algorithm}
\caption{\textit{Diameter}($\gamma$) }\label{alg:diameter}
%\begin{minipage}{1.5\columnwidth}
\begin{multicols}{2}
\begin{algorithmic}[1]

\State $c_{old},q,r,b \gets$ first point of the stream
\State $c_{new} \gets$ null
\For {all element $p$ of the stream}
\If {$c_{old}$ is deleted}
\If {$c_{new} \neq $null and $c_{old} = q$}
\State $c_{old} \gets r$; $b \gets c_{new}$;
\State $c_{new} \gets $ null; 
\EndIf
\If {$c_{new} \neq $null and $c_{old} \neq q$}
\State $b \gets c_{old}$; $c_{old} \gets q$;
\State $c_{new} \gets $ null;
\EndIf
\If {$c_{new} = $null}
\State $b \gets c_{old}$; $c_{old} \gets r$;
\EndIf
\EndIf
\State INSERT($p$)
\State $r \gets p$
\EndFor

\Procedure{INSERT}{a}
\If {$c_{new} =$ null}

\If {$|pr| > \gamma$}
\State $c_{old}$,$q \gets r$; $c_{new} \gets p$;
%\EndIf
\ElsIf {$|pc_{old}| > \gamma$}
%\If {$|pc_{old}| > \gamma$}
\State $q \gets r$; $c_{new} \gets p$;
\EndIf
\Else
\If {$|pr| > \gamma$}
\State $c_{old}$,$q \gets r$; $c_{new} \gets p$;

%\Else
\ElsIf {$|pc_{new}| > \gamma$}
\State $c_{old} \gets c_{new}$; $q \gets r$; $c_{new} \gets p$;
%\EndIf
%\Else
\ElsIf {$|pq| > \gamma$}
\If {$c_{old} \neq q$}
\State $c_{old} \gets q$; $q \gets r$; $c_{new} \gets p$;
\EndIf
\EndIf
\EndIf
%\EndIf

\EndProcedure
\end{algorithmic}
\end{multicols}
\end{algorithm}

First we give $(6+\epsilon)$-approximation by using the algorithm for the diameter problem. The algorithm of Cohen-Addad et al.~\cite{cohen-2016} returns two points $p$ and $q$ such that its distance is at least $\frac{(1-\epsilon)}{3}|\textit{Dia}(P_N)|$. We choose the center as the last point and the radius as $3|pq|$. We give an example that $(6+\epsilon)$-approximation. See the figure~\ref{fig:onecenter} (a).

Now we explain $(3+\epsilon)$-approximation. Our idea in this section is to carefully adapt the algorithm 1 of Cohen-Addad et al.~\cite{cohen-2016}, originally designed for the diameter problem. We call our algorithm $Diameter(\gamma)$. To improve readability, we sketch their algorithm and its properties to explain our modifications.

Their algorithm composes of two parts: a fixed parameter algorithm and a way to maintain parameters.

Given an estimate $\gamma$ they maintain four points $c_{old}$, $c_{new}$, $q$, and $r$, where $q$ is immediately prior to $c_{new}$ and $r$ is the most recent point. Their algorithm returns either two points $c_{old}$ and $c_{new}$ ($\textit{Time}(c_{old}) < \textit{Time}(c_{new})$) such that $|c_{old}c_{new}| \ge \gamma$ or a point $c_{old}$.
$\textit{Diameter}(\gamma)$ is almost the same with their algorithm except maintaining a bridge point $b$. We will explain $b$ later.
%They have two invariants and show that the invariants are satisfied during their algorithm \textcolor{red}{is running}. 
They show that the following two invariants are satisfied.
The invariants are:
\begin{invariant}
\label{inv:1}
If $c_{new} = null$ then the following statements hold: \\
a) For any alive points $x,y$ with $\textit{Time}(x), \textit{Time}(y) \le \textit{Time}(c_{old})$, we have $|xy| \le 2\gamma$.	\\
b) For any point $x$ with $\textit{Time}(x) > \textit{Time}(c_{old})$, we have $|xc_{old}| \le \gamma$.
\end{invariant}

\begin{invariant}
\label{inv:2}
If $c_{new} \neq null$, then the following statements hold:	\\
a) $|c_{old}c_{new}| > \gamma$.	\\
b) For any point $x$ with $\textit{Time}(c_{old}) < \textit{Time}(x) < \textit{Time}(c_{new})$, we have $|xc_{old}| \le \gamma$.	\\
c) For any point $x$ with $\textit{Time}(c_{new}) < \textit{Time}(x)$, we have $|xc_{new}| \le \gamma$.	\\
d) If $c_{old} \neq q$ then for any point $x$ with $\textit{Time}(q) < \textit{Time}(x)$, we have $|xq| \le \gamma$.
\end{invariant}

Now we explain some properties that are used later and you can easily ckeck the correctness of the properties in the paper of Cohen-Addad et al.~\cite{cohen-2016}.
If $\textit{Diameter}(\gamma)$ returns a point, then $3\gamma \ge |\textit{Dia}(P_N)|$ by Invariant 1.
Their algorithm returns $c_{old} = p_{n-1}$ and $c_{new} = p_n$ if $|p_{n-1}p_n| > \gamma$.
If $\gamma > |\textit{Dia}(P_N)|$, then returning a point $c_{old}=r$ is satisfying Invariant 1.

They maintain estimates, which is an exponential sequence to the base of ($1+\epsilon$), such that any value between the distance of the closest pair and the distance of the diameter is ($1+\epsilon$) approximated. For each power of ($1+\epsilon$), they run their algorithm.
They choose the largest estimate $\gamma$ such that $\textit{Diameter}(\gamma)$ returns two points $c_{old}$ and $c_{new}$.
%They show that $|Dia(P_N)| \le 3\gamma$.
Note that $\textit{Diameter}(\gamma (1+\epsilon))$ returns a point and its means $3\gamma (1+\epsilon) \ge |\textit{Dia}(P_N)|$ by Invariant 1.

To adapt this idea to $1$-center problem, we add an invariant. %to modify their algorithm.
This invariant is a variant of the Invariant 1 and is given in the proofs of their Lemma 3 and Lemma 4.

\begin{lemma}[Invariant 3]
\label{inv:3}
If $c_{new} = null$ then the following statement holds:	\\
For any alive point $x$ with $\textit{Time}(x) \le \textit{Time}(c_{old})$, there exists a bridge point $b$ such that $|xb| \le \gamma$.
\end{lemma}
\begin{proof}
We consider the situation when Invariant 3 holds and a new point $p$ is inserted. We will show that Invariant 3 is satisfied after the update.
%how to update their algorithm when a new point $p$ is inserted.
Let $c'_{old}$ ($c'_{new}$) be the point $c_{old}$ ($c_{new}$) before $p$ is inserted. Let $r'$, $q'$ and $b'$ be defined similar way.
%before their algorithm update the points.

There are 3 cases when $c_{new}=null$ and $b \neq b'$. You can easily ckeck this in the paper of Cohen-Addad et al.~\cite{cohen-2016}. \\
%the bridge point $b$ is changed. \\
Case 1 : $c'_{new} = null$ and $c'_{old}$ is deleted. 		\\
Case 2 : $c'_{new} \neq null$ and $c'_{old} = q$, and $c'_{old}$ is deleted.	\\
Case 3 : $c'_{new} \neq null$ and $c'_{old} \neq q$, and $c'_{old}$ is deleted.

We explain how to update the bridge point $b$ for each case. Note that for any case $c'_{old}$ is deleted.\\
\textbf{Case 1)} In this case, their algorithm sets $c_{old} = r'$. We need to show that for any point $x$ with $\textit{Time}(c'_{old}) < \textit{Time}(x) \le \textit{Time}(r')= \textit{Time}(c_{old})$, there is a point $b$ such that $|xb| \le \gamma$. By Invariant 1.b), for any point $x$ with $\textit{Time}(c'_{old}) < \textit{Time}(x) \le \textit{Time}(r')$, we have $|c'_{old}x| \le \gamma$. We set $b = c'_{old}$.	\\
\textbf{Case 2)} In this case, their algorithm sets $c_{old} = r'$. We need to show that for any point $x$ with $\textit{Time}(c'_{old}) < \textit{Time}(x) \le \textit{Time}(r')= \textit{Time}(c_{old})$, there is a point $b$ such that $|xb| \le \gamma$. Since $c'_{old} = q$ and $\textit{Time}(q) = \textit{Time}(c'_{new})-1$, $c'_{new}$ is the oldest alive point. And, by Invariant 2.c), for any point $x$ with $\textit{Time}(c'_{new}) \le \textit{Time}(x) \le \textit{Time}(r')$, we have $|xc'_{new}| \le \gamma$. We set $b = c'_{new}$.	\\
\textbf{Case 3)} In this case, their algorithm sets $c_{old} = q'$. We need to show that for any point $x$ with $\textit{Time}(c'_{old}) < \textit{Time}(x) \le \textit{Time}(q') < \textit{Time}(c'_{new})$, there is a point $b$ such that $|xb| \le \gamma$. By Invariant 2.b), for any point $x$ with $\textit{Time}(c'_{old}) < \textit{Time}(x) = \textit{Time}(c_{old}) < \textit{Time}(c'_{new})$, we have $|xc'_{old}| \le \gamma$. We set $b = c'_{old}$.
\end{proof}

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.8\textwidth]{figures/onecenter}
	\caption{(a) $p$ and $q$ are diameter and $|pq| = 2 r^*$. Therefore $3|pq| \le 6 r^*$ (b) $B(m,1.5\gamma)$ contains $P_N$}
	\label{fig:onecenter}
\end{figure}

Now we explain how to modify their algorithm.
In $\textit{Diameter}(\gamma)$ we maintain a bridge point b.

In our algorithm, we choose the smallest estimate $\gamma$ such that $\textit{Diameter}(\gamma)$ returns a point $c_{old}$.
%They show that $|Dia(P_N)| \le 3\gamma$.
Note that $\textit{Diameter}(\frac{\gamma}{1+\epsilon})$ returns two points and its means $\frac{\gamma}{1+\epsilon} \le |\textit{Dia}(P_N)|$. Since $|\textit{Dia}(P_N)| \le 2\rst$, therefore $\gamma \le 2(1+\eps)\rst$.
%Their algorithm maintains many estimates and chooses the smallest $\gamma'$ that returns a point $c_{old}$. We choose $\gamma=\frac{\gamma'}{(1+\eps)}$ Since they have an estimate and it returns two points and a diameter is at most $2\rst$, we have $\gamma \le (2+\eps)\rst$. 
By Invariant 1 and Invariant 3, for any alive point $x$, we have $|xb| \le \gamma$ or $|xc_{old}| \le \gamma$. Since $|bc_{old}| \le \gamma$, we choose the mid point $m$ of $b$ and $c_{old}$. Then for any alive point $x$ $|xm| \le 1.5 \gamma$. We give a ball $B(m,1.5\gamma)$ as our solution. Since $\gamma \le 2(1+\eps)\rst$, it guarantees $(3+3\eps)$-approximation. See Figure~\ref{fig:onecenter} (b).
%By setting $\epsilon' = \epsilon/3$ and running our algorithm with $\epsilon'$, we get a ($3+\epsilon$)-approximation.
Because we have one more point per estimate than their algorithm, the space complexity of both algorithms is the same.
%our algorithm is the same with the space complexity of their algorithm.

Now we explain the way to bound the number of estimates.
Let $\Upsilon$ be an estimates set containing $(1+\eps)^i $ for all integer $i$. See the Figure~\ref{fig:bound_region}.
We modify some solutions of their algorithm such that the new solutions also satisfy all invariants. We define $\gamma_L$ and $\gamma_U$ as follows. 
Let $\gamma_L$ ($\gamma_U$) be an estimate in $\Upsilon$ such that for any estimate $\gamma  \le \gamma_L$ ($\gamma_U \le \gamma$) the solution of their algorithm for $\gamma$ is the same solution of the algorithm for $\gamma_L$ ($\gamma_U$). 
By this property, we know all the solutions in $\Upsilon$ by just maintaining estimates between $\gamma_L$ and $\gamma_U$.

To find proper $\gamma_L$ and $\gamma_R$, we use evidences.

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.8\textwidth]{figures/boundR}
	\caption{$\gamma_L$ and $\gamma_U$ and their evidences}
	\label{fig:bound_region}
\end{figure}

\begin{lemma}
	If $\gamma \le |p_{n-1}p_n|$, then $\textit{Diameter}(\gamma)$ returns a solution $c_{old} = r = p_{n-1}$ and $c_{new} = p = p_n$.
	If $\gamma > |\textit{dia}(P_N)|$, then we can return a point $c_{old} = r$ and all the invariants hold for the solution.
\end{lemma}
\begin{proof}
	First we prove the case when $\gamma \le |p_{n-1}p_n|$. In their algorithm, if $\gamma \le |p_{n-1}p_n|$ then their algorithm set $c_{old}= p_{n-1}$ and $c_{new} = p_n$ as the solution. We use the same result, therefore all invariants hold.
		
Now we prove the case when $\gamma > |\textit{dia}(P_N)|$. When $\gamma > |\textit{dia}(P_N)|$, we set $c_{old}$, $r$ and $q$ to $p_{n-1}$, $c_{new} = null$ and $b = p_{n-1}$. Note that Invariant 1 and Invariant 3 hold because $\gamma > |\textit{dia}(P_N)|$.
\end{proof}

We set $\gamma_L < |p_{n-1}p_n|$. Let $\gamma_{e}$ be the length of their solution. Because their solution is a $(3+\eps)$-approximation for the diameter problem, we set $\gamma_U = 3(1+\epsilon)\gamma_{e}$ and it is larger than the length of the diameter.
%Note that finding $\gamma_L$ is simple, but finding $\gamma_U$ is more difficult because finding the diameter is difficult. However, the solution of their algorithm is a $(3+\eps)$-approximation for the diameter problem, so we use the length of the solution. Let be $\gamma_{e}$ the length. We choose a $\gamma_U$ that is larger then $3\gamma_{e}$.

When a constant number of points are inserted, we maintain all estimates between $\gamma_L$ and $\gamma_U$ by using evidences for each direction.
Then we update $\gamma_L$ and $\gamma_U$. We first update the direction decreasing the number of estimates if it is possible.
%To update $\gamma_{min}$, if $dist(r,p) < \gamma_{min}$, we set the largest  estimate $\gamma = (\frac{1}{1+\eps})^i\gamma_{min} \le dist(r,p)$ to new $\gamma_{min}$ where $i$ is a positive integer. Otherwise find the largest $\gamma'$ such that the solution for $\gamma$ is the same with the solution for $\gamma_{min}$ $\forall \gamma \le \gamma'$. We set $\gamma_{min} = \gamma'$.
%To update $\gamma_{max}$, if $dist(r,p) \ge \gamma_{max}$, we set the smallest  estimate $\gamma = (1+\eps)^i\gamma_{man} \ge dist(r,p)$ to new $\gamma_{max}$ where $i$ is a positive integer. Otherwise find the smallest $\gamma'$ such that the solution for $\gamma$ is the same with the solution for $\gamma_{max}$ $\forall \gamma \ge \gamma'$. We set $\gamma_{max} = \gamma'$.
Because $\gamma_L$ is larger than $|CP(P_N)|$ and $\gamma_U$ is smaller than $3|\textit{Dia}(P_N)|$, the number of estimates is bounded by the same complexity with their algorithm.

Therefore we obtain at the following Theorem.

\begin{theorem}
\label{thm:1-center}
	Given a set of points $P$ with a window of size $N$ and a value $\epsilon > 0$, our algorithm guarantees a $(3+\eps)$-approximation to the Euclidean $1$-center problem in the sliding window model using O$(\log(\alpha)/\epsilon)$ space and update time in arbitrary dimensions $d$.
\end{theorem}

%Note that our algorithm returns $3$-approximation of the cost of the $1$-center problem.

==> includes/1-center_new.tex <==
\section{The 1-Center Problem}
\label{section:1-center}


\begin{algorithm}
\caption{\textit{Diameter}($\gamma$) }\label{alg:diameter}
%\begin{minipage}{1.5\columnwidth}
\begin{multicols}{2}
\begin{algorithmic}[1]

\State $c_{old},q,r,b \gets$ first point of the stream
\State $c_{new} \gets$ null
\For {all elements $p$ of the stream}
\If {$c_{old}$ is deleted}
\If {$c_{new} \neq $null and $c_{old} = q$}
\State $c_{old} \gets r$; $b \gets c_{new}$;
\State $c_{new} \gets $ null; 
\EndIf
\If {$c_{new} \neq $null and $c_{old} \neq q$}
\State $b \gets c_{old}$; $c_{old} \gets q$;
\State $c_{new} \gets $ null;
\EndIf
\If {$c_{new} = $null}
\State $b \gets c_{old}$; $c_{old} \gets r$;
\EndIf
\EndIf
\State INSERT($p$)
\State $r \gets p$
\EndFor

\Procedure{INSERT}{p}
\If {$c_{new} =$ null}

\If {$|pr| > \gamma$}
\State $c_{old}$,$q \gets r$; $c_{new} \gets p$;
%\EndIf
\ElsIf {$|pc_{old}| > \gamma$}
%\If {$|pc_{old}| > \gamma$}
\State $q \gets r$; $c_{new} \gets p$;
\EndIf
\Else
\If {$|pr| > \gamma$}
\State $c_{old}$,$q \gets r$; $c_{new} \gets p$;

%\Else
\ElsIf {$|pc_{new}| > \gamma$}
\State $c_{old} \gets c_{new}$; $q \gets r$; $c_{new} \gets p$;
%\EndIf
%\Else
\ElsIf {$|pq| > \gamma$}
\If {$c_{old} \neq q$}
\State $c_{old} \gets q$; $q \gets r$; $c_{new} \gets p$;
\EndIf
\EndIf
\EndIf
%\EndIf

\EndProcedure
\end{algorithmic}
\end{multicols}
\end{algorithm}

First we give a $(6+\epsilon)$-approximation by using the algorithm for the diameter problem.
%논문 찾아보자.
The metric diameter problem is to find two points of maximum distance among a set of points lying in some metric space.
The algorithm of Cohen-Addad et al.~\cite{cohen-2016} returns two points $p$ and $q$ such that their distance is at least $\frac{(1-\epsilon)}{3}|\textit{Dia}(P_N)|$. We choose the last point as the center and $3|pq|$ as the radius. We give an example that gives $(6+\epsilon)$-approximation. See Figure~\ref{fig:onecenter} (a). In the figure, the length of the diameter is $2r^*$.

Now we explain our $(3+\epsilon)$-approximation algorithm. Our idea in this section is to carefully adapt Algorithm 1 of Cohen-Addad et al.~\cite{cohen-2016}, originally designed for the diameter problem. To improve readability, we sketch their algorithm and its properties to explain our modifications.
Their algorithm consists of two parts: a fixed parameter algorithm and a way to maintain parameters. We only explain the first part.

For a given estimate $\gamma$, their algorithm maintains four points $c_{old}$, $c_{new}$, $q$, and $r$.
%, where $q$ is immediately prior to $c_{new}$ and $r$ is the most recent point.
Their algorithm returns either two points $c_{old}$ and $c_{new}$ ($\textit{Time}(c_{old}) < \textit{Time}(c_{new})$) such that $|c_{old}c_{new}| \ge \gamma$ or a point $c_{old}$. If their algorithm returns one point, then they show that $|Dia(P_N)| \le 3 \gamma$ in this case.

They show that the following two invariants are satisfied.
The invariants are:
\begin{invariant}
\label{inv:1}
If $c_{new} = null$ then the following statements hold: \\
a) For any alive points $x,y$ with $\textit{Time}(x), \textit{Time}(y) \le \textit{Time}(c_{old})$, we have $|xy| \le 2\gamma$.	\\
b) For any point $x$ with $\textit{Time}(x) > \textit{Time}(c_{old})$, we have $|xc_{old}| \le \gamma$.
\end{invariant}

\begin{invariant}
\label{inv:2}
If $c_{new} \neq null$, then the following statements hold:	\\
a) $|c_{old}c_{new}| > \gamma$.	\\
b) For any point $x$ with $\textit{Time}(c_{old}) < \textit{Time}(x) < \textit{Time}(c_{new})$, we have $|xc_{old}| \le \gamma$.	\\
c) For any point $x$ with $\textit{Time}(c_{new}) < \textit{Time}(x)$, we have $|xc_{new}| \le \gamma$.	\\
d) If $c_{old} \neq q$ then for any point $x$ with $\textit{Time}(q) < \textit{Time}(x)$, we have $|xq| \le \gamma$.
\end{invariant}

Now we explain our algorithm. Our algorithm consists of two parts: a fixed parameter algorithm and a way to maintain parameters.

Given an estimate $\gamma$, we use their fixed parameter algorithm with maintaining  a new point. 
%We will explain \textit{bridge} point later. 
We call our algorithm $Diameter(\gamma)$.
We maintain a \textit{bridge} point and following an invariant show the property of the point. The main idea is that two balls $B(c_{old},\gamma)$ and $B(b,\gamma)$ contain all alive point if our algorithm returns a point $c_{old}$ where $b$ is a bridge point. See Figure~\ref{fig:onecenter} (b).
This invariant is a variant of the Invariant 1 and is given implicitly in the proofs of their Lemma 3 and Lemma 4~\cite{cohen-2016}.

\begin{lemma}[Invariant 3]
\label{inv:3}
If $c_{new} = null$ then the following statement holds:	\\
There exists a \textit{bridge} point $b$ such that $|xb| \le \gamma$ for any alive point $x$ with $\textit{Time}(x) \le \textit{Time}(c_{old})$.
\end{lemma}
\begin{proof}
We consider the situation when Invariant 3 holds and a new point $p$ is inserted. We will show that Invariant 3 is satisfied after the update.
%how to update their algorithm when a new point $p$ is inserted.
Let $c'_{old}$ ($c'_{new}$) be the point $c_{old}$ ($c_{new}$) before $p$ is inserted. Let $r'$, $q'$ and $b'$ be defined similar way.
%before their algorithm update the points.

There are 3 cases when $c_{new}=null$ and $b \neq b'$. \\
%You can easily ckeck this in the paper of Cohen-Addad et al.~\cite{cohen-2016}. \\
%the bridge point $b$ is changed. \\
Case 1 : $c'_{new} = null$ and $c'_{old}$ is deleted. 		\\
Case 2 : $c'_{new} \neq null$ and $c'_{old} = q$, and $c'_{old}$ is deleted.	\\
Case 3 : $c'_{new} \neq null$ and $c'_{old} \neq q$, and $c'_{old}$ is deleted.

We explain how to update the bridge point $b$ for each case. Note that for any case $c'_{old}$ is deleted.\\
\textbf{Case 1)} In this case, their algorithm sets $c_{old} = r'$. We need to show that for any point $x$ with $\textit{Time}(c'_{old}) < \textit{Time}(x) \le \textit{Time}(r')= \textit{Time}(c_{old})$, there is a point $b$ such that $|xb| \le \gamma$. By Invariant 1.b), for any point $x$ with $\textit{Time}(c'_{old}) < \textit{Time}(x) \le \textit{Time}(r')$, we have $|c'_{old}x| \le \gamma$. We set $b = c'_{old}$.	\\
\textbf{Case 2)} In this case, their algorithm sets $c_{old} = r'$. We need to show that for any point $x$ with $\textit{Time}(c'_{old}) < \textit{Time}(x) \le \textit{Time}(r')= \textit{Time}(c_{old})$, there is a point $b$ such that $|xb| \le \gamma$. Since $c'_{old} = q$ and $\textit{Time}(q) = \textit{Time}(c'_{new})-1$, $c'_{new}$ is the oldest alive point. And, by Invariant 2.c), for any point $x$ with $\textit{Time}(c'_{new}) \le \textit{Time}(x) \le \textit{Time}(r')$, we have $|xc'_{new}| \le \gamma$. We set $b = c'_{new}$.	\\
\textbf{Case 3)} In this case, their algorithm sets $c_{old} = q'$. We need to show that for any point $x$ with $\textit{Time}(c'_{old}) < \textit{Time}(x) \le \textit{Time}(q') < \textit{Time}(c'_{new})$, there is a point $b$ such that $|xb| \le \gamma$. By Invariant 2.b), for any point $x$ with $\textit{Time}(c'_{old}) < \textit{Time}(x) = \textit{Time}(c_{old}) < \textit{Time}(c'_{new})$, we have $|xc'_{old}| \le \gamma$. We set $b = c'_{old}$.
\end{proof}

By Invariant 1 and 3, we can find a solution.

\begin{lemma}
\label{small_ball}
If $c_{new} = null$ then $B(m,1.5\gamma)$ contains $P_N$ where $m = \frac{c_{old}+b}{2}$.
\end{lemma}
\begin{proof}
By Invariant 3, we have a \textit{bridge} point $b$, for any alive point $x$ that is older than $c_{old}$, satisfying $|xb| \le \gamma$. By Invariant 1, $|xc_{old}| \le \gamma$ for any $x$ with $Time(x) > Time(c_{old})$. $|bc_{old}| \le \gamma$ by Invariant 3. We choose the mid point $m$ of $b$ and $c_{old}$. Then for any alive point $x$ $|xm| \le 1.5 \gamma$. See Figure~\ref{fig:onecenter} (b).%We give a ball $B(m,1.5\gamma)$ as our solution.
\end{proof}

Now we explain the way to maintain estimates. First we explain the case when the number of estimate is unbounded and then we explain the case when the number of estimate is bounded.

We maintain estimates, which is an exponential sequence to the base of ($1+\epsilon$), such that any value between the distance of the closest pair and the distance of the diameter is ($1+\epsilon$) approximated. For each power of ($1+\epsilon$), we run $\textit{Diameter}(\gamma)$.

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.6\textwidth]{figures/onecenter}
	\caption{(a) $p$ and $q$ are diameter and $|pq| = 2 r^*$. Therefore $3|pq| \le 6 r^*$ (b) $B(m,1.5\gamma)$ contains $P_N$}
	\label{fig:onecenter}
\end{figure}

Now we explain the way to bound the number of estimates.
Let $\Upsilon$ be an estimates set containing $(1+\eps)^i $ for all integer $i$. See the Figure~\ref{fig:bound_region}.
We modify some solutions of our algorithm such that the new solutions also satisfy all invariants and maintain the specific points.
% We define $\gamma_L$ and $\gamma_U$ as follows. 
Let $\gamma_L$ ($\gamma_U$) be an estimate in $\Upsilon$ such that, for any estimate $\gamma  \le \gamma_L$ ($\gamma \ge \gamma_U$),  $Diameter(\gamma)$ and $Diameter(\gamma_L)$ ($Diameter(\gamma_U)$) maintain the same points and the same solution.
By this property, we know all the solutions in $\Upsilon$ by just maintaining estimates between $\gamma_L$ and $\gamma_U$.

%To find proper $\gamma_L$ and $\gamma_R$, we use evidences.
To find proper $\gamma_L$ and $\gamma_U$, we use the following witnesses.

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.6\textwidth]{figures/boundR}
	\caption{$\gamma_L$ and $\gamma_U$ and their witnesses}
	\label{fig:bound_region}
\end{figure}

\begin{lemma}
%invariant 및 유지하는 정보들도 같다는걸 보영야 한다.
	If $\gamma \le |p_{n-1}p_n|$, then $\textit{Diameter}(\gamma)$ maintains $c_{old},r,q \gets p_{n-1}$ and $c_{new} \gets p_n$. It returns $c_{old}$ and $c_{new}$ as a solution.
	If $\gamma > |\textit{dia}(P_N)|$, then we can maintain $c_{old}$, $r$, $q 
\gets p_{n-1}$, $c_{new} \gets null$ , and $b \gets p_{n-1}$. We return $c_{old}$ as a solution. All the invariants hold for the solution.
\end{lemma}
\begin{proof}
	First we prove the case when $\gamma \le |p_{n-1}p_n|$.
	% In their algorithm, if $\gamma \le |p_{n-1}p_n|$ then their algorithm set $c_{old}= p_{n-1}$ and $c_{new} = p_n$ as the solution. We use the same result, therefore all invariants hold.
	After updating $p_{n-1}$, we set $r$ to $p_{n-1}$ by line 14 of Algorithm 1. When $p_n$ is inserted our algorithm call \textit{Insert}$(p)$. In the procedure, whether $c_{new}$ is null or not, $|pr| > \gamma$. So we set $c_{old}$ and $q$ to $r$ and $c_{new}$ to $p$. Since $c_{new}$ is not null, we do not maintain $b$. In line 14, we set $r$ to $p_n$.  
		
		
When $\gamma > |\textit{dia}(P_N)|$, we set $c_{old}$, $r$ and $q$ to $p_{n-1}$, $c_{new}$ to null, and $b$ to $p_{n-1}$. Note that Invariant 1 and Invariant 3 hold because $\gamma > |\textit{dia}(P_N)|$.
\end{proof}

We set the largest estimate satisfying $\gamma < |p_{n-1}p_n|$ as $\gamma_L$. Let $\gamma_{e}$ be the length of our solution. Because $\gamma_e \ge |Dia(P_N)|/3$ by Invariant 1, we set the smallest estimate satisfying $\gamma \ge 3\gamma_{e}$ as $\gamma_U$.
%Note that finding $\gamma_L$ is simple, but finding $\gamma_U$ is more difficult because finding the diameter is difficult. However, the solution of their algorithm is a $(3+\eps)$-approximation for the diameter problem, so we use the length of the solution. Let be $\gamma_{e}$ the length. We choose a $\gamma_U$ that is larger then $3\gamma_{e}$.

When a constant number of points are inserted, we maintain all estimates between $\gamma_L$ and $\gamma_U$ by using evidences for each direction.
Then we update $\gamma_L$ and $\gamma_U$. We first update the direction decreasing the number of estimates if it is possible.
%To update $\gamma_{min}$, if $dist(r,p) < \gamma_{min}$, we set the largest  estimate $\gamma = (\frac{1}{1+\eps})^i\gamma_{min} \le dist(r,p)$ to new $\gamma_{min}$ where $i$ is a positive integer. Otherwise find the largest $\gamma'$ such that the solution for $\gamma$ is the same with the solution for $\gamma_{min}$ $\forall \gamma \le \gamma'$. We set $\gamma_{min} = \gamma'$.
%To update $\gamma_{max}$, if $dist(r,p) \ge \gamma_{max}$, we set the smallest  estimate $\gamma = (1+\eps)^i\gamma_{man} \ge dist(r,p)$ to new $\gamma_{max}$ where $i$ is a positive integer. Otherwise find the smallest $\gamma'$ such that the solution for $\gamma$ is the same with the solution for $\gamma_{max}$ $\forall \gamma \ge \gamma'$. We set $\gamma_{max} = \gamma'$.
Because $\gamma_L$ is larger than $|CP(P_N)|$ and $\gamma_U$ is smaller than $3|\textit{Dia}(P_N)|$, the number of estimates is $O(\log_{1+\eps}\alpha) = O(\frac{\log \alpha}{\log (1+\eps)}) = O(  \log (\alpha)/\eps)$.

Among estimates, we choose the smallest estimate $\gamma$ that $\textit{Diameter}(\gamma)$ returns a point $c_{old}$.
Note that $\textit{Diameter}(\frac{\gamma}{1+\epsilon})$ returns two points and its means $\frac{\gamma}{1+\epsilon} \le |\textit{Dia}(P_N)|$. Since $|\textit{Dia}(P_N)| \le 2\rst$, $\gamma \le 2(1+\eps)\rst$. Therefore our solution $B(m,1,5\gamma)$ guarantees $(3+3\eps)$-approximation. See Figure~\ref{fig:onecenter} (b).

Note that $\textit{Diameter}(\gamma)$ takes a constant time to update.

Therefore we obtain the following Theorem.

\begin{theorem}
\label{thm:1-center}
	Given a set of points $P$ with a window of size $N$ and a value $\epsilon > 0$, our algorithm guarantees a $(3+\eps)$-approximation to the Euclidean $1$-center problem in the sliding window model maintaining O$(\log(\alpha)/\epsilon)$ points and requiring update time per point in arbitrary dimensions $d$.
\end{theorem}

==> includes/algorithm.tex <==
\section{Upper bound}

==> includes/conclusion.tex <==
\section{Conclusion}\label{section:conclusion}
We have shown non-trivial bounds for the problem of enclosing a fire in the upper half-plane by an infinite horizontal \wall.
Our results show that delaying barriers---in this case vertical segments attached to the \wall from above---can help to break the obvious upper bound of~2 for the building speed.
It will be interesting to see if such an effect can also be achieved for the problem of containing the fire by a closed barrier curve, \ie, for Bressan's original problem.


==> includes/introduction.tex <==
\section{Introduction and problem statement}
The k-center problem, which is finding $k$ smallest congruent balls containing a set of input points, is a fundamental problem arising from abundant real-world applications, including machine learning, data mining, and image processing. The growth of the Internet and the computing power of machines has facilitated an increase in the amount of data collected and used by various applications has significantly increased over the last decades. But in huge data sets it is quite hard to guarantee reasonable processing time and memory space. To cope with this difficulty, data stream models have received considerable attention in the theoretical as well as the application field.

In the streaming model, it is important to design an algorithm whose space complexity does not depend on the size of the input, since the memory size is typically much smaller than the input size. In this paper, we consider the single-pass streaming model~\cite{chan-pathak-2014}, where elements in the data stream are allowed to be examined only once and only a limited amount of information can be stored. The insertion-only stream model is well studied, but also more flexible settings like dynamic streams and the sliding window model have received some attention for many clustering problems. In the dynamic stream model input points can be removed arbitrarily and in the sliding window model older input is deleted as new elements arrive.

%c 5 T. M. Chan and V. Pathak. Streaming and dynamic algorithms for minimum enclosing balls in high dimensions. Comput. Geom. Theory Appl., 47(2):240–247, 2014.


In this paper, we consider the Euclidean $k$-center problem for a sliding window, which contains the most recent $N$ points. 


\subsection{Previous Work}
%a  2
%b	1.8
%c	outlier
%d	sliding window

\textbf{The $k$-center problem in the static setting}.
The Euclidean $k$-center problem has been extensively studied in the literature.
If $k$ is part of the input, the $k$-center problem is $\mathrm{NP}$-hard~\cite{garey-johnson-1979}, even in the plane~\cite{megiddo-supowit-1984}.
In fact, it is known to be $\mathrm{NP}$-hard to approximate the $k$-center problem with a factor smaller than $2$ for arbitrary metric spaces~\cite{fowler-paterson-1981}, and with a factor smaller than $1.822$ for the Euclidean space~\cite{bern-eppstein-1996}.
If the Euclidean dimension $d$ is not fixed, the problem is $\mathrm{NP}$-hard for fixed $k \ge 2$~\cite{megiddo-1990}. Agarwal and Procopic~\cite{agarwal-procopiuc-2002} gave an exact algorithm that runs in O$(n^{k^{1-(1/d)}}$) for the $L_2$-metric and the $L_{\infty}$-metric.
Feder and Greene~\cite{feder-greene-1988} gave a $2$-approximation algorithm that runs in O($n \log k$) for any $L_p$-metric.


%a3. P. K. Agarwal and C. M. Procopiuc, Exact and approximation algorithms for clustering, Algorithmica 33 (2002) 201–226.

%a6. M. Bern and D. Eppstein, Approximation algorithms for geometric problems, Approximation Algorithms for NP-Hard Problems (PWS Publishing Co., 1996).

%a15. D. Feder and D. H. Greene, Optimal algorithms for approximate clustering, Proc. 20th Annu. ACM Symp. Theory of Computing (1988), pp. 434–444.

%a16. M. R. Garey and D. S. Johnson, Computers and Intractability: A Guide to the Theory of NP-Completeness (W.H. Freeman, New York, 1979).

%a23. M. Megiddo, On the complexity of some geometric problems in unbounded dimension, J. Symbolic Comput. 10 (1990) 327–334.

%a24. M. Megiddo and K. J. Supowit, On the complexity of some common geometric location problems, SIAM J. Comp. 13(1) (1984) 182–196.

%c10 R. J. Fowler, M. S. Paterson, and S. L. Tanimoto. Optimal packing and covering in the plane are NP-complete. Inform. Process. Lett., 12(3):133–137, 1981.

%[7] B. Chazelle and J. Matouˇsek. On linear-time deterministic algorithms for optimization problems in fixed dimension. J. Algorithms, 21(3):579–597, 1996.


For small k and d, better solutions are available. The $1$-center problem in fixed dimensions is known to be of LP-type and can be solved in linear time~\cite{chazelle-matousek-2015}.
For the Euclidean $2$-center problem in the plane, the best known algorithm is given by Chan~\cite{chan-1999}, which runs deterministically in O($n \log^2 n \log^2 \log n$) time using O($n$) space. \\
%If k is fixed, Kim and Ahn~\cite{kim-ahn-2015} gave an $(1.8+\eps)$-approximation using O($1/\eps$) space. If $d$ and $k$ are fixed, Zarrabi-Zadeh~\cite{zarrabi-2008} gave an $(1+\eps)$-approximation algorithm using O($k(1/\eps)^d$) space. \\
\textbf{The $k$-center problem in the streaming model}.
In the streaming model, where only a single pass over the input is allowed, McCutchen and Khuller~\cite{mccutchen-khuller-2008} and independently Guha~\cite{guha-2009} presented algorithms to maintain a $(2 + \eps)$-approximation for $k$-centers in any dimension using O($(kd/\eps) \log(1/\eps)$) space. For $k = 1$, Zarrabi-Zadeh and Chan~\cite{zarrabi-chan-2006} presented a simple algorithm achieving an approximation factor of $3/2$ using only O($d$) space. Agarwal and Sharathkumar~\cite{agarwal-shara-2010} improved the approximation factor to $(1 + \sqrt{3})/2 + \eps \approx 1.37$ using O($(d(1/\eps)^3) \log(1/\eps)$) space. The approximation factor of their algorithm was later improved to $1.22$ by Chan and Pathak~\cite{chan-pathak-2014}. For $k = 2$, Kim and Ahn~\cite{kim-ahn-2015} gave a $(1.8 + \eps)$-approximation using O($d/\eps$) space. Their algorithm extends to any fixed $k$, with the same approximation factor.
If $d$ and $k$ are fixed, Zarrabi-Zadeh~\cite{zarrabi-2008} gave an $(1+\eps)$-approximation using O($k(1/\eps)^d$) space. \\
In the sliding window model, Cohen-Addad et al.~\cite{cohen-2016} have recently obtained results for a variant of the $k$-center problem that returns only $k$ points. 
Under the assumption that the algorithm cannot create new points, they show that any randomized sliding window algorithm achieving
an approximation factor less than 4 with probability greater than $1/2$
for metric 2 center problem requires $\Omega(\sqrt[3]{N})$ points.
For $k=2$, they give a $(4+\eps)$-approximation using O($1/\eps \log \alpha)$ where $\alpha$ is the ratio of the largest and smallest distance and is assumed to be known in advance. For general $k$, they gave a $(6+\eps)$-approximation maintaining O($1/\eps \log \alpha)$ points. \\
\textbf{Problems in the sliding window model}.
Many problems have been studied in the literature~\cite{braverman-ostrovsky-2010,braverman-2016}. Diameter problem are studied~\cite{feigenbaum-2004,chan-Sadjad-2006,cohen-2016}. Chan and Sadjad~\cite{chan-Sadjad-2006} give a $(1+\epsilon)$-approximation using $O((1/\epsilon)^{(d+1)/2}\log \alpha / \epsilon)$ points. For higher dimensions, Cohen-Addad et al.~\cite{cohen-2016} give a $(3+\epsilon)$-approximation maintaining $O(1/\epsilon \log \alpha)$ points.

%braverman-ostrovsky-2010
%braverman-2016

%Feigenbaum-2004
%chan-Sadjad-2006
%Joan Feigenbaum, Sampath Kannan, and Jian Zhang. Computing diameter in the streaming and sliding-window models. Algorithmica, 41(1):25–41, 2004.

%Timothy M. Chan and Bashir S. Sadjad. Geometric optimization problems over sliding
%windows. Int. J. Comput. Geometry Appl., 16(2-3):145–158, 2006.


%[2] P. K. Agarwal and R. Sharathkumar. Streaming algorithms for extent problems in high dimensions. In Proc. 21st ACM-SIAM Sympos. Discrete Algorithms, pages 1481–1489, 2010.
%[13] S.-S. Kim and H.-K. Ahn. An improved data stream algorithm for clustering. Comput. Geom. Theory Appl., 48(9):635–645, 2015.

%[17] H. Zarrabi-Zadeh and T. M. Chan. A simple streaming algorithm for minimum enclosing balls. In Proc. 18th Canad. Conf. Computat. Geom., pages 139–142, 2006

%[12] S. Guha. Tight results for clustering and summarizing data streams. In Proc. 12th Internat. Conf. Database Theory, pages 268–275, 2009.

%15] R. M. McCutchen and S. Khuller. Streaming algorithms for k-center clustering with outliers and with anonymity. In Proc. 11th Internat. Workshop Approx. Algorithms, pages 165–178, 2008.

\subsection{Technical Contribution}
For the $1$-center problem, we introduce a point that reduces the approximation factor of our algorithm. Moreover we remove the assumption that $\alpha$ is known in advance by modifying some solutions.

For the $k$-center problem, we find a coreset of size $O(k)$, which guarantees $(c+2\sqrt{3}+\epsilon)$-approximation by using $c$-approximation for the coreset.
\textcolor{blue}{
A coreset is a small portion of the data, such that running a clustering algorithm on it, generates a clustering for the whole data, which is approximately optimal.}
We use the observation that no three points within the Euclidean unit ball have all pairwise distance more than $\sqrt{3}$.

%k-center low D
For the $k$-center in low dimension, we use a property of doubling metric space recursively. While our idea seems intuitive, it has, to our knowledge, not been used before
in this context
%To our knowledge, this idea is not published, however this idea is too intuitive. So we believe this idea is already known.
\subsection{Our Contribution}

%For the $1$-center problem, we give a $(3+\eps)$-approximation in the sliding window model that maintains O($1/\eps \log \alpha$) points and update time per point, where $\alpha$ is the ratio of largest and smallest possible distance between the points. But alpha need not be known in advance.

For the $1$-center problem we obtain a $(3+\epsilon)$-approximation that works without knowing aspect ratio $\alpha$ in advance, by adding a carefully chosen point. Our algorithm maintains O($1/\eps \log \alpha$) points and update time per point, where $\alpha$ is the ratio of largest and smallest possible distance between the points.


In the static model, finding a $2$-approximation for the $1$-center problem is known and easy, however, in the streaming model finding a $\textit{feasible}$ radius is difficult because we do not know all the points. Therefore our result is not trivial. 


For the $k$-center problem, our algorithm finds a coreset of size $O(k)$ maintaining O($k/\eps \log \alpha$) points and O($k \log k + k/\eps \log \alpha$) update time per point. 
Our algorithm gives a $(c+2\sqrt{3} + \epsilon)$-approximation algorithm for the Euclidean $k$-center problem by using any given $c$-approximation for the coreset where $c$ is a positive real number.
For small $k$, we give a $(1+2\sqrt{3} + \eps)$-approximation  ($\approx 4.465$) using O$(k^{k^{1-(1/d)}}$) time per point. For large $k$, we give a $(2+2\sqrt{3} + \eps)$-approximation ($\approx 5.465$) using $O(k\log k)$ time per point. Our two algorithms for $k$-center problem are an improvement on the approximation factor of $(6+\eps)$ by Cohen-Addad et al.~\cite{cohen-2016} with the same space complexity.
We also remove the assumption that $\alpha$ is known in advance.
It is important to remove the assumption for implementing an algorithm in the streaming model.
\textcolor{blue}{
Our idea is general enough to be adapted to the algorithms of Cohen-Addad et al. for the metric diameter problem and the metric $k$-center problem.}


For low dimensional Euclidean space, better approximation is available. 
Our algorithm finds a coreset of size $O(k)$ maintaining O($k2^{c_d t} \log(\alpha)/\epsilon$) points and \textcolor{blue}{hoho} update time per point where $t$ is an arbitrary positive integer and $c_d$ is a constant related with doubling dimension. 
We give a $(c+2\sqrt{3}(\frac{1}{2})^t+\epsilon)$-approximation by using any given $c$-approximation for the coreset. We can get $(1+\epsilon)$-approximation by using this result.
%We give a $(1+\eps)$-approximation using O($k(1/\eps)^d \log(\alpha)/\epsilon$) space.
This result breaks the lower bound of Cohen-Addad et al.~\cite{cohen-2016} in low dimensional Euclidean spaces. The idea breaks the lower bound of the diameter problem in low dimensional Euclidean spaces.

~\\
The rest of this paper is organized as follows.
Section~\ref{section:preliminaries} formally introduces the problem as well as terms and definitions required for the analysis.
In Section~\ref{section:1-center} we give an approximation algorithm for the Euclidean $1$-center problem and show a way to remove the assumption that $\alpha$ is given in advance.
In Section~\ref{section:k-center} we give an approximation algorithm for the Euclidean $k$-center problem.
In Section~\ref{section:k-center_low} we give an approximation algorithm for the Euclidean $k$-center problem in low dimension. 

==> includes/k-center_lowD.tex <==
\section{The k-Center Problem in Low Dimension}
\label{section:k-center_low}

In this section, \textcolor{red}{we explain better approximations} when the dimension of Euclidean space is low. In Section~\ref{section:k-center_low_double}, we give an $(1+2(\frac{\sqrt{3}}{2})^t+\eps)$-approximation algorithm using O($k2^{c_d d t} \log(\alpha)/\epsilon$) space where $t$ is a positive integer. In Section~\ref{section:k-center_low_grid}, we give an $(1+\eps)$-approximation algorithm using O($k(1/\eps)^d \log(\alpha)/\epsilon$) space.

\subsection{\texorpdfstring{$(1+2(\frac{\sqrt{3}}{2})^t+\eps)-$}{Lg}approximation algorithm}
\label{section:k-center_low_double}
In this section, we use a property of doubling metric space.
The doubling dimension~\cite{assouad-1983,heinonen-2001} of a metric space is the smallest $D$ such that every ball of radius $r$ is covered by $2^D$ balls of radius most $r/2$. It is well-known that a point set in $d$-dimensional Euclidean metric has doubling dimension $\Theta (d)$. In~\cite{verger-2005}, Jean-Louis give a constant $c_d$ ( equation (4) in Theorem 1.2) such that $D \le c_dd$.

%[3] P. Assouad. Plongements lipschitziens dans R n . Soci´et´e math´ematique de France, 111:429–448, 1983. 

%[12] J. Heinonen. Lectures on analysis on metric spaces. Universitext. Springer New York, 2001.

%[??] Jean-Louis Verger-Gaugry: Covering a Ball with Smaller Equal Balls in Rn. Discrete & Computational Geometry 33(1): 143-155(2005)
\begin{table}[ht]
\caption{Relation between the approximation factor and the number of balls} % title of Table
\centering % used for centering table
\begin{tabular}{c c c } % centered columns (4 columns)
\hline\hline %inserts double horizontal lines
$t$     & APX 			& balls \\ [0.5ex] % inserts table
%heading
\hline % inserts single horizontal line
1 		& $2.733+\eps$	& O($2^{c_d d}$) 		\\
3 		& $1.434+\eps$	& O($2^{3c_d d}$) 		\\
5 		& $1.109+\eps$	& O($2^{5c_d d}$) 		\\
8 		& $1.014+\eps$	& O($2^{8c_d d}$) 		\\
10 		& $1.004+\eps$	& O($2^{10c_d d}$) 		\\ [1ex] % [1ex] adds vertical space
\hline %inserts single line
\end{tabular}
\label{table:nonlin} % is used to refer this table in the text
\end{table}

A unit ball is contained in $2^{c_dd}$ balls with radius $1/2$. We can use this idea recursively. A ball with radius $1/2$ is contained in $2^{c_dd}$ balls with radius $(1/2)^2$. Therefore $2^{(c_dd)t}$ balls with radius $(1/2)^t$ contain a unit ball.
By lemma~\ref{lem:2ball_cotain}, a ball with radius $(1/2)^t$ is contained in the union of two balls with radius $\sqrt{3}(1/2)^t$.

%\textcolor{red}{However we cannot use this idea directly because the result means there exist such balls \textcolor{red}{not abitrary}. We use the same approach in Section~\ref{section:k-center}. Let $B$ be a ball with $(1/2)^t$. By Lemma~\ref{lem:2ball_cotain}, for any points $c_1$ and $c_2$ such that $c_1$, $c_2 \in B$ and $dist(c_1,c_2) > \sqrt{3}(1/2)^t$, $B \subset B(c_1,\sqrt{3}(1/2)^t) 
%\cup B(c_2,\sqrt{3}(1/2)^t)$.} Therefore a ball with radius $(1/2)^t$ is contained by any two balls whose center in the ball and radius is $\sqrt{3}(1/2)^t$.

The basic idea of our algorithm is similar with our algorithm in Section~\ref{section:k-center}. The difference is that we maintain a set $A$ of at most $2^{(c_dd)t}$ active center points and the distance between a active center point and its representative point is at most $\sqrt{3}(1/2)^tr$.
%By changing Algorithm 1 the following way, we have a result. We maintain $2^{(c_dd)t}$ active center points, and set radius to $\sqrt{3}(1/2)^tr$. By similar reason,
If $\rst < r \le (1+\eps) \rst$, then our algorithm returns \textit{feasible} solution and it guarantees a $(1+2\sqrt{3}(\frac{1}{2})^t+\epsilon)$-approximation.
To bound the number of estimates, we set $r_L < \frac{|CP(P_{2^{(c_dd)t}+1})|}{\sqrt{3}}$ and $r_U = \frac{2|dia(P_N)|}{\sqrt{3}}$.
\begin{theorem}
\label{thm:lowD_doubling}
	Given a set of points $P$ with a window of size $N$, a value $\eps > 0$ and a fixed dimention $d$, our algorithm guarantees a $(1+2\sqrt{3}(\frac{1}{2})^t+\epsilon)$-approximation to the Euclidean $k$-center problem in the sliding window model using O$(k2^{c_d d t} \log(\alpha)/\epsilon)$ space and update time.
\end{theorem}

In Table $1$, we summarize the relation between the approximation factor and the number of balls for some value $t$.
% add table



\subsection{\texorpdfstring{$(1+\eps)-$}{Lg}approximation algorithm}
\label{section:k-center_low_grid}

%21. H. Zarrabi-Zadeh, Core-preserving algorithms, Proc. 20th Canadian Conf. Computational Geometry (2008), pp. 159–162.

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.6\textwidth]{figures/grid}
	\caption{A Grid example.}
	\label{fig:grid}
\end{figure}

Our $(1+\eps)$-approximation algorithm is an adaptation of an algorithm by Zarabi-Zadeh~\cite{zarrabi-2008}.
To improve readability, we sketch their algorithm, then we explain our algorithm.

Let $\mathsf{g}_s$ be a uniform grid of side length $s$. Note that the length of the diameter of a grid cell is $\sqrt{d}s$. For each non-empty cell we maintain a last inserted point. We call those points a coreset. Let $\mathcal{B} = \{B_1, \ldots , B_k \} $ be an optimal solution for the coreset. Then we enlarge the balls by $\sqrt{d}s$. Note that all input points lie in the union of the enlarged balls. To compute $(1+\epsilon)$-approximation we set $s \le \epsilon / \sqrt{d} r^*$. The size of a coreset is $O(k(1/\epsilon))^d$ and update time for a inserted point is $O(1)$.

We modify above algorithm to use in the sliding window model. Let $c_d$ be the maximum number of cells that have an intersect with an optimal ball. If the number of points in a coreset exceed $kc_d$, then we remove oldest point and set our coreset is \textit{infeasible} until the removed point is not alive.

Now we explain our algorithm. Given an estimate optimal radius r, our algorithm maintains a coreset by $\mathsf{g}_{\epsilon / \sqrt{d} r}$. we maintain estimates, which is an exponential sequence to the base of ($1+\epsilon$), such that any value between $r_L$ and $r_U$ approximated. For each power of ($1+\epsilon$), we run our algorithm.

%For a given estimate radius $r$. We maintain a uniform grid of side length $\eps r/\sqrt{d}$ implicitly. Note that the length of the diameter is at most $\eps r$. (See the Figure~\ref{fig:grid}.) When a new point arrives, we maintain the cell containing the point. Let $c_d$ be constant such that a ball with radius r intersects with at most $c_d$ cells of the grid. The number of cells we maintain can exceed $c_dk$. Then we maintain $c_dk$ cells \textcolor{red}{that point is arrived lately} and set this solution as 
%\textit{infeasible} until the removed points are deleted. We find the smallest $k$ balls containing the cells, and it guarantees $(1+\eps)$-approximation.

%We ﬁrst explain the subroutine in the plane and then show how to extend it for higher dimensions. Given an estimate length $l$


%The algorithm maintains an axis-parallel rectangle $R$ and a dc/εe×dc/εe grid over R, where c = 24√2.Let h(R) and w(R) denote the height and the width of R, respectively. The side-lengths of a grid cell are proportional to the side-lengths of R, that is, the height and the width of a grid cell are h(R)/dc/εe and w(R)/dc/εe, respectively.

To bound the number of estimates, we use similar idea in Section~\ref{section:k-center}. We set $r_L$ such that last $kc_d+1$ points lie in the different cells. 
It takes O($kc_d \log (kc_d)$) time by the algorithm of Feder and Greene~\cite{feder-greene-1988}. Note that $r_L$ is bounded by a constant times the length of the closest pair and can make a coreset for $r \le r_L$ if we know last $kc_d$ points in $P_N$. We set $r_U$ such that all points in $P_N$ lies in a cell. Note that $r_U$ is bounded by a constant times the length of the diameter.

\begin{theorem}
\label{thm:lowD_grid}
	Given a set of points $P$ with a window of size $N$, a value $\eps > 0$ and a fixed dimension $d$, our algorithm guarantees a $(1+\eps)$-approximation to the Euclidean $k$-center problem in the sliding window model using O$(k(1/\eps)^d \log(\alpha)/\epsilon)$ space and update time.
\end{theorem}

\begin{ackn}
We thank all anonymous referees for their valuable input.
We thank Rolf Klein, David Kübel, Elmar Langetepe and Barbara Schwarzwald	for their valuable discussion.
\end{ackn}

==> includes/lowerBound.tex <==
\section{A lower bound of \ensuremath{v>1.5}}
First, we show that not all possible \crewss have to be considered.

\begin{lemma}[Increasing \wall lengths]
	\label{lem:increasing-walls}
	For any \crews $\mathcal{S}$ viable for a speed $v$, there exists a \crews consisting of vertical \walls of strictly increasing length in each direction which is also viable for $v$.	
	That is, $\B_{i +1} > \B_i$ and $\D_{i+1} > \D_i$, $\forall i \geq 1$.
\end{lemma}

\begin{proof}
	Assume $\mathcal{S}$ contains a vertical \wall $w_2$ that is at most as long as the previous one $w_1$ in that direction.
	Then consider the \crews $\mathcal{S}' = \mathcal{S} \setminus {w_2}$.
	Removing $w_2$ does not decrease the shortest $L_1$ path from the \fire origin $(0,0)$ to any point in the plane including points on all other \walls, as those paths are prolonged by $w_1$.
	However, $w_2$ is no longer consumed and hence the total \burn $\BF{\mathcal{S'}}(t) \leq \BF{\mathcal{S}}(t)$ for all $t$ and therefore $\QF{\mathcal{S}'}(t) \leq \QF{\mathcal{S}}(t)$.
\end{proof}

\begin{theorem}[Lower Bound]
	\label{thm:lowerbound}
	There exists no viable \crews for any speed $v \leq 1.5$.
\end{theorem}

\begin{proof}
The idea of the proof is to show that the ratios \consumptionRatio[l,r] are always larger than $0.5$, for $t$ greater than some threshold and sometimes exceed $1$ for arbitrarily large $t$.
We start with the latter.

Assume there exists a \crews $\mathcal{S}^{*}$ which is viable for $v<1.5$.
For every time $t_0 > 0$ there must exist some point in time $t_1 > t_0$, where the current \burn is at most $1$.
Because the current consumption takes on integer values, it would otherwise be greater or equal than $2$ all the time, requiring speed $v\geq 2$.
Hence, at $t_1$ at least for one of the directions the current \burn is $0$.
This can only happen if the fire burns along the back of a vertical \wall and has fully consumed all \walls previously touched in this direction.
For example, such a $0$-interval can be seen at $d_2$ in \autoref{fig:baseExample}.

\Wlog assume this happens on the left-hand side.
By Lemma~\ref{lem:increasing-walls}, we can also assume that \walls are strictly increasing in length in both directions.
Consider the time $t$ and total \burn $\BF{\mathcal{S}^{*}}^l(t)$ in the left direction at the beginning of a $0$-interval.
\begin{center}
	$t 	 =   \sum\limits_{k=1}^i \A_k + \B_i + \max(0, 2 \B_{i-1} - \B_i)$ \quad\quad\quad
	$\BF{\mathcal{S}^{*}}^l(t)  =  \sum\limits_{k=1}^i \A_k + \sum\limits_{k=1}^i \B_k -  \startWall$
\end{center}
For an explanation of the $\max(0, 2 \B_{i-1} - \B_i)$ summand, see \autoref{fig:0-interval-start}.
\begin{figure}[ht]
	\centering
	\includegraphics[height=3cm,page=1]{figures/0-interval-beginningAlternative}
	\caption{
		The two possible configurations at the beginning of a $0$-interval at time $t$. 
		In the first case, the \fire reached the lower end of the $\B_{i}$ \wall first, so the $0$-interval starts exactly when the upper end is reached.
		In the second case, the upper end was reached first, so the $0$-interval begins when the lower end is reached after additional time $2 \B_{i-1} - \B_i$.
	}
	\label{fig:0-interval-start}
\end{figure}

Assume \,$\QF{\mathcal{S}^{*}}^l(t) \leq 1$, then $\frac{\BF{\mathcal{S}^{*}}^l(t)}{t} \leq 1$ and $\BF{\mathcal{S}^{*}}^l(t) \leq t$
\begin{equation*}
\def\arraystretch{2}
\begin{array}{l r c l }
\Rightarrow 	
	& \sum\limits_{k=1}^i \A_k + \sum\limits_{k=1}^i \B_k - \startWall 
	&\leq 
	& \sum\limits_{k=1}^i \A_k + \B_i + \max(0, 2 \B_{i-1} - \B_i) \\
	%\Leftrightarrow \sum\limits_{k=1}^i \B_k  &> \B_i + \max(0, 2 \B_{i-1} - \B_i) + \startWall \\
\Rightarrow 
	& \sum\limits_{k=1}^{i-2} \B_k + \B_{i-1} + \B_{i}
	& \leq
	& \max( \B_i, 2 \B_{i-1}) + \startWall
\end{array}
\end{equation*}
Due to Lemma~\ref{lem:increasing-walls} $\B_{i-1} + \B_{i} > \max(\B_i, 2 \B_{i-1})$ and $\sum_{k=1}^{i-2} \B_k > (i-2) \cdot \B_1 > \startWall$ for $i$ larger than some threshold $i_0$.
As the left-hand current \burn is $0$ for arbitrarily large $t$, we can assume $i>i_0$.
But this is a contradiction.
Hence $\QF{\mathcal{S}^{*}}^l(t) > 1$ at the beginnings of all $0$-intervals after some threshold $t_0$ in the left-hand direction.

Hence for the whole \crews $\mathcal{S}^{*}$ to be viable for $v<1.5$, the \ratio $\QF{\mathcal{S}^{*}}^r(t)$ in the right-hand direction must be below $0.5$ at exactly these moments.
Hence for the right-hand direction $0$-intervals exist for arbitrarily large $t$.

The ends of those $0$-intervals are local minima of that directions \ratio.
Consider the time $t$ and total \burn $\BF{\mathcal{S}^{*}}^r(t)$ in the right-hand direction at the end of such an interval.
\begin{center}
	$ t = \sum\limits_{k=1}^i \C_k + \D_i + \min(\C_{i+1}, \D_i) $ \quad\quad\quad $\BF{\mathcal{S}^{*}}^r(t) = \sum\limits_{k=1}^i \C_k + \sum\limits_{k=1}^i \D_k - \startWall$
\end{center}
For an explanation of the $\min(\C_{i+1}, \D_i)$ summand, see \autoref{fig:0-interval-end}.
\begin{figure}[ht]
	\centering
	\includegraphics[height=3cm,page=1]{figures/0-interval-endAlternative}
	\caption{
		The two possible configurations at the end of a $0$-interval at time $t$. 
		In the first case, the $0$-interval ends, when the \fire reaches the highway, $\D_i$ time units after passing the top of the $\D_i$ \wall.
		In the second case, the next \wall is reached before the highway, so the $0$-interval ends, $\C_{i+1}$ time units after passing the top of the $\D_i$ \wall.
	}
	\label{fig:0-interval-end}
\end{figure}

Assume $\QF{\mathcal{S}^{*}}^r(t) < 0.5$, then $\frac{\BF{\mathcal{S}^{*}}^r(t)}{t} < 0.5$ and $2 \cdot \BF{\mathcal{S}^{*}}^r(t) < t$
\begin{equation*}
\begin{array}{l r c l}
\Rightarrow
	& 2 \cdot \sum\limits_{k=1}^i \C_k + 2 \cdot \sum\limits_{k=1}^i \D_k - 2 \startWall
	& <
	& \sum\limits_{k=1}^i \C_k + \D_i + \min(\C_{i+1}, \D_i) \\
\Rightarrow
	& \sum\limits_{k=1}^i \C_k + 2 \cdot \sum\limits_{k=1}^i \D_k  
	& <
	& 2 \D_i  + 2 \startWall
\Rightarrow \sum\limits_{k=1}^i \C_k + 2 \cdot \sum\limits_{k=1}^{i-1} \D_k < 2 \startWall
\end{array}
\end{equation*}

As above $\sum_{k=1}^{i-1} \D_k > (i-1) \D_1 > 2 \startWall$ for $i$ larger than some threshold $i_0$.
Hence after some threshold time $t_0$, even at the local minima the \ratio of the right-hand direction is above $0.5$, hence it is always above $0.5$.
Therefore $\QF{\mathcal{S}^{*}}(t)$ exceeds $1.5$ for arbitrarily large~$t$, which makes $\mathcal{S}^*$ not viable for $v \leq 1.5$.
\end{proof}


==> includes/lowerBoundZiWi.tex <==
\newcommand{\useful}{helpful\xspace}
\section{Lower bounds}
\label{section:lowerBounds}
Observe that a vertical barrier which is shorter than the predecessor in the same direction does not delay the fire.
Hence, we assume that vertical barriers strictly increase in length in both directions.

Let us consider the \burn intervals.
We know that $0$-intervals are repeatedly necessary in at least one of the directions, else the \ratio will converge to $2$.
\Wlog let this be the right direction.

Let $z_i$ denote the $i$-th $0$-interval in this direction.
Between two consecutive $0$-intervals $z_i$ and $z_{i+1}$, there is a sequence of $k$-intervals with $k\geq1$.
However, the exact composition of these $k$-intervals depends on the \crews.
To circumvent this, we refer to this whole sequence of $k$-intervals by $w_i$.
Together we refer to such a pair $(z_i$, $w_i)$ as the cycle $i$. 
For simplicity, let $w_i$ and $z_i$ also denote the length of these intervals.

Let $t_i = \sum_{j=1}^{i-1} (w_j + z_j)$ denote the start time of $z_i$, \ie the beginning of cycle $i$.
%Equivalently for the other direction, let $y_h$ denote the $0$-intervals and $v_h$ the interval between two $0$-intervals.
%TODO search for maximum ?
%TODO check if resorting is really not used
%\Wlog regarding a lower bound, we can assume the $k$-intervals within one $w_i$ are sorted ascending by $k$, as this never increases total \burn and hence \ratio at any point $t$.
Let $w_{i,k}$ be the total length of all $k$-intervals within $w_i$ and $K_i$ be the largest $k$ within $w_i$ with $w_{i,k} > 0$.
Then, let $W_i^\mu = \sum_{k=1}^{K_i} k \cdot w_{i,k}$ denote the total consumption during $w_i$.
This is equal to the consumption $\BF{}^r(t_i, t_{i+1})$ during the whole cycle $i$ as there is no consumption during the $0$-interval $z_i$.

We can derive the following fundamental observations: %for $i>2$
\begin{lemma}
	\label{lem:axioms}
	\textbf{i)} The consumption during $w_i$ is higher than the lengths of the previous and the next  $0$-interval combined, so $W_i^\mu \geq z_i + z_{i+1}$.
	\textbf{ii)} During $w_i$ there are $k$-intervals with $k\geq 2$ for a duration of at least $z_i$, so $z_i \leq w_i - w_{i,1} \leq w_i$.
\end{lemma}

\begin{proof}
%	Each $z_i$ %except the very first stemming from the buffer
%	happens while the fire burns along the back of a vertical barrier of some length $b_j$, and will end when the fire reaches the $x$-axis or the next vertical barrier, so $z_i \leq \min(a_{j+1}, b_j) < a_{j+1}$.\\
	Let $b_i$ be the length of the delaying barrier generating $z_i$ and $a_{i+1}$ the distance to the next vertical delaying barrier of length $b_{i+1}$ in the same direction.
	Then, $z_i \leq \min(a_{i+1}, b_i)$.\\
	\textbf{i)} The next $0$-interval $z_{i+1}$ will be generated by some delaying barrier of length $b_k$ with $k > i$, so $z_{i+1} \leq b_k$.
	However, both $a_{i+1}$ and $b_k$ (and possibly additional barriers) must be consumed completely before the next $0$-interval can begin, but have not been reached by the fire before $w_i$, hence $W_i^\mu \geq a_{i+1} + b_k \geq z_i + z_{i+1}$.\\
	\textbf{ii)} Consider the time $t$, when the fire reaches the lower endpoint of $b_{i+1}$, which lies somewhere within $w_i$. 
	Then between $t - \min(a_{i+1}, b_{i})$ and $t$ the fire burns along the both, the $x$-axis and the next delaying barrier $b_{i+1}$.
	This means we have at least a $2$-interval for duration $\min(a_{i+1}, b_i) \geq z_i$.
\end{proof}
Note that this formally holds only for $i \geq 2$ due to the headstart barrier.
However, it can be shown that all following conclusions hold after some threshold time $t_0$, depending on the headstart length \startWall.
As we are constructing a lower bound for local maxima, this does not affect the actual lower bound.

\begin{lemma}
\label{lem:local-maxima}
At the beginning of a $0$-interval %$z_i$, \ie at $t_i$,
the \ratio %$\mathcal{Q}^r(t_i)$ 
in that direction exceeds~$1$. %, i.e. $\mathcal{Q}(t_i) \geq 1$. 
\end{lemma}
\begin{proof}
%\Wlog we consider a $0$-interval $z_i$ in the right direction.
%Within each cycle, the consumption $W_i^\mu$ exceeds the duration $z_i + w_i$, as
%	$ W_i^\mu = \sum_{k=1}^{K_i} k \,w_{i,k} = \sum_{k=1}^{K_i} w_{i,k} + \sum_{k=1}^{K_i} (k-1) w_{i,k}$
By definition, $\sum_{k=1}^{K_i} w_{i,k} = w_i$ and, by Lemma \ref{lem:axioms} $ii)$, $\sum_{k=1}^{K_i} (k-1) w_{i,k} \geq \sum_{k=2}^{K_i} w_{i,k} = w_i - w_{i,1} \geq z_i$.
It follows that
\[
\QF{}^r(t_i)
	= \frac{\sum\limits_{j=1}^{i-1} W_j^\mu}{\sum\limits_{j=1}^{i-1} (z_j + w_j)} 
	= \frac{\sum\limits_{j=1}^{i-1} \left(\sum\limits_{k=1}^{K_j} (k-1) w_{j,k} + \sum\limits_{k=1}^{K_j} w_{j,k}\right)}{\sum\limits_{j=1}^{i-1} (z_j + w_j)}
	\geq 1.
\]
\end{proof}
%
Lemma~\ref{lem:local-maxima} also implies that there must be $0$-intervals repeatedly in both directions.
%
\begin{lemma}
\label{lem:local-minima}
At the end of a $0$-interval %$z_i$, i.e. at $t_i + z_i$, 
the \ratio %$\mathcal{Q}^r(t_i + z_i)$ 
in that direction exceeds $\nicefrac{1}{2}$. %, i.e. $\mathcal{Q}(t_i + z_i) \geq \nicefrac{1}{2}$.
As local minima with a ratio below $1$ can only appear at the end of a $0$-interval, this implies that  the \ratio in one direction exceeds $\nicefrac{1}{2}$ at all times $t$.
\end{lemma}
%
\begin{proof}
Consider a $0$-interval $z_i$, which ends at time $t_i +  z_i$.
Then,
\begin{equation*}
	\def\arraystretch{2}
	\begin{array}{rr l }
		&t_i + z_i &= \sum\limits_{j=1}^{i-1} (w_j + z_j) + z_i = \sum\limits_{j=1}^{i-1} w_j + \sum\limits_{j=1}^{i-2} z_j + (z_{i-1} + z_i) \\
		&& \overset{\text{Le.\ref{lem:axioms}}}{\leq} \sum\limits_{j=1}^{i-1} w_j + \sum\limits_{j=1}^{i-2} w_j + W_{i-1}^\mu
			\leq \sum\limits_{j=1}^{i-1} W_j^\mu + \sum\limits_{j=1}^{i-2} W_j^\mu + W_{i-1}^\mu 
			\leq 2 \sum\limits_{j=1}^{i-1} W_j^\mu \\[1em]
		\Leftrightarrow & \frac{1}{2} &\leq \frac{\sum\limits_{j=1}^{i-1} W_j^\mu}{t_i + z_i} = \mathcal{Q}^r(t_i + z_i).
	\end{array}
	\end{equation*}
\end{proof}
%
\begin{corollary}
Lemma \ref{lem:local-maxima} and Lemma \ref{lem:local-minima} together imply that at least $v \geq 1.5$ is necessary.
\end{corollary}
%
Now assume there exists a \crews for a speed $v = 1.5 + \varepsilon$, so $\sup_t \QF{}(t)< \nf{3}{2} + \varepsilon$.
%Let's consider only situations after the threshold $t$ for which the above lemma holds.
%
Let $(z_i$, $w_i)$ be a cycle during which a cycle from the other direction ends.
Let us call such a cycle a {\em \useful cycle} as its minimum is used to counter the high consumption at the end of a cycle in the other direction.
Then the local minimum at the end of $z_i$, \ie at $t_i + z_i$, must attain a ratio below $\nicefrac{1}{2} + \varepsilon$, hence
\begin{equation*}
\QF{}(t_i + z_i) = \frac{\sum\limits_{j=1}^{i-1} W_j^\mu}{z_i + t_i} \leq \nicefrac{1}{2} + \varepsilon 
\quad \Leftrightarrow \quad \sum\limits_{j=1}^{i-1} W_j^\mu \leq  \left(z_i + t_i\right)\left(\nicefrac{1}{2} + \varepsilon\right).
\end{equation*}
%
We also know the following for $t_i$ from Lemma \ref{lem:local-maxima}:
\begin{equation*}
\QF{}(t_i) = \frac{\sum\limits_{j=1}^{i-1} W_j^\mu}{t_i} \geq 1 
\quad \Leftrightarrow \quad 
 \sum\limits_{j=1}^{i-1} W_j^\mu \geq t_i.
\end{equation*}
%
Combining this we get:
\begin{equation}
\label{ineq:1}
\def\arraystretch{1.5}
\begin{array}{l r c l }
& &t_i &\leq \left(z_i + t_i\right)\left(\nicefrac{1}{2} + \varepsilon\right) \\
& \Leftrightarrow &t_i \left(\nicefrac{1}{2}- \varepsilon\right) &\leq z_i \left(\nicefrac{1}{2}+ \varepsilon\right) \\
& \Leftrightarrow & \sum\limits_{j=1}^{i-1} \left( w_j + z_j \right) &\leq \frac{\nicefrac{1}{2}+ \varepsilon}{\nicefrac{1}{2} - \varepsilon} \cdot z_i
%& \Leftrightarrow & z_i &\geq \frac{\nicefrac{1}{2}- \varepsilon}{\nicefrac{1}{2} + \varepsilon} \sum\limits_{j=1}^{i-1} \left( w_j + z_j \right)
\end{array}
\end{equation}
This proves the following lemma.
\begin{lemma}
\label{lem:helpfulZi}
For helpful cycles $i$, we have
$z_i \geq \frac{\nicefrac{1}{2}- \varepsilon}{\nicefrac{1}{2} + \varepsilon} \sum_{j=1}^{i-1} \left( w_j + z_j \right)$.
\end{lemma}
The unique local minimum of a \useful cycle $i$ attains a \ratio between $\nicefrac{1}{2}+\varepsilon$ and $\nicefrac{1}{2}$.
Let $[t_i + z_i - l_i, t_i + z_i + r_i]$ be the interval around the minimum at $t_i + z_i$, where the \ratio in that direction is below or equal to $\nicefrac{1}{2}+\varepsilon$, as illustrated in \autoref{fig:r-intervals}.
To keep the global ratio below $\nf{3}{2}+\varepsilon$, the end of the cycle in the other direction must lie in this interval.
\begin{figure}[ht]
	\centering
	\includegraphics[width=.6\textwidth]{figures/r-interval}
	\caption{A local minimum in a helpful cycle.}
	\label{fig:r-intervals}
\end{figure}

We know for $t_i + z_i$ by \autoref{lem:local-minima} that $\mathcal{C}^r(t_i + z_i) \geq \nicefrac{1}{2} (t_i + z_i)$.
There also is at least \burn $1$ between $t_i + z_i$ and $t_i + z_i + r_i$, as it is part of $w_i$, hence:
\begin{equation*}
	\nicefrac{1}{2} + \varepsilon = \frac{\mathcal{C}^r(t_i + z_i + r_i)}{t_i + z_i + r_i} \geq \frac{\mathcal{C}^r(t_i + z_i) + r_i}{t_i + z_i + r_i} 
	\geq \frac{\nf{1}{2} \cdot (t_i + z_i) + r_i}{t_i + z_i + r_i}.
\end{equation*}
%
Solving this inequality for $r_i$ yields
\begin{equation}
\label{ineq:r-t}
	r_i \leq \frac{\varepsilon}{\nicefrac{1}{2} - \varepsilon} (t_i + z_i) = \frac{\varepsilon}{\nicefrac{1}{2} - \varepsilon} \left(\sum\limits_{j=1}^{i-1} \, (z_j + w_j) + z_i\right).
\end{equation}
%
By Lemma \ref{lem:helpfulZi}, $r_i$ can be related directly to $z_i$:
\begin{equation}
\label{ineq:r}
r_i \leq \frac{\varepsilon}{\nicefrac{1}{2} - \varepsilon} \left(\frac{\nicefrac{1}{2} + \varepsilon}{\nicefrac{1}{2} - \varepsilon} \, z_i + z_i\right) = \frac{\varepsilon}{\left(\nicefrac{1}{2} - \varepsilon\right)^2} \, z_i .
\end{equation}
%
Equivalently, applying the fact, that there is consumption $0$ between $t_i + z_i -l_i$ and $t_i + z_i$, yields a bound for $l_i$:
\begin{equation}
\label{ineq:l}
l_i \leq \frac{\varepsilon}{\nicefrac{1}{2} + \varepsilon} (t_i + z_i) = \frac{\varepsilon}{\nicefrac{1}{2} - \varepsilon} \left(\sum\limits_{j=1}^{i-1}(z_j + w_j) + z_i\right) \leq \frac{\varepsilon}{\left(\nicefrac{1}{2} - \varepsilon\right) \left(\nicefrac{1}{2} + \varepsilon\right)} \, z_i.
\end{equation}
%
\begin{lemma}
\label{lem:rl-interval}
In a helpful cycle $i$ we have the following for $r_i$ and $l_i$ as defined above:
\begin{equation*}
\def\arraystretch{1.2}
\begin{array}{l}
l_i \leq \frac{\varepsilon}{\nicefrac{1}{2} + \varepsilon} (t_i + z_i) \leq \frac{\varepsilon}{\left(\nicefrac{1}{2} - \varepsilon\right) \left(\nicefrac{1}{2} + \varepsilon\right)} \, z_i \\

r_i \leq \frac{\varepsilon}{\nicefrac{1}{2} - \varepsilon} \left(t_i + z_i\right) \leq \frac{\varepsilon}{\left(\nicefrac{1}{2} - \varepsilon\right)^2} \, z_i.
\end{array}
\end{equation*}

\end{lemma}
From Lemma \ref{lem:local-minima} it follows that the \ratio in one direction can attain values of at most $1 + \varepsilon$.
But that does not mean that the \ratio of a single cycle (so $\nf{\mathcal{C}(t_i,t_{i+1})}{(z_i + w_i)}$) is at most $1 + \varepsilon$.
However, the \ratio of a cycle can not be arbitrarily large, as the \ratio is greater than $1$ at the beginning of the cycle and at most $1 + \varepsilon$ at the end.
Assume a single cycle has a \ratio of $1 + \beta \varepsilon$, so:
\begin{equation}
\label{eq:worst-cycle-duration}
	\frac{\mathcal{C}(t_i,t_{i+1})}{z_i + w_i}
	= 1 + \beta \varepsilon 
	\quad \Leftrightarrow \quad \mathcal{C}(t_i,t_{i+1}) = (z_i + w_i) (1 + \beta \varepsilon)
\end{equation}
%
%For the beginning of the cycle it holds:
%\begin{equation}
%\label{eq:worst-cycle-start}
%\frac{\mathcal{C}(t_{i})}{t_{i}} \geq 1 
%\quad\Leftrightarrow\quad 
%\mathcal{C}(t_{i}) \geq t_i
%\end{equation}
%
Now consider the ratio at the end of the cycle:
\begin{equation*}
\def\arraystretch{2}
\begin{array}{l r c l }
&\frac{\mathcal{C}(t_{i+1})}{t_{i+1}} &= \frac{\mathcal{C}(t_{i}) + \mathcal{C}(t_i, t_{i+1})}{t_i + z_i + w_i} &\leq 1 + \varepsilon \\
\Leftrightarrow && \mathcal{C}(t_{i}) + \mathcal{C}(t_i, t_{i+1}) &\leq (t_i + z_i + w_i) (1 + \varepsilon).
\end{array}
\end{equation*}
%
Applying Lemma \ref{lem:local-maxima} and \autoref{eq:worst-cycle-duration} yields:
\begin{equation*}
\def\arraystretch{1.5}
\begin{array}{c r l }
&t_i + (z_i + w_i)(1+ \beta \varepsilon) &\leq (t_i + z_i + w_i) (1 + \varepsilon)\\
\Leftrightarrow &t_i + (z_i + w_i) + (z_i + w_i)\beta \varepsilon &\leq t_i + (z_i + w_i) + t_i \varepsilon + (z_i + w_i) \varepsilon \\
\Leftrightarrow &(z_i + w_i)\beta \varepsilon &\leq t_i \varepsilon + (z_i + w_i) \varepsilon \\
\Leftrightarrow &(z_i + w_i)( \beta -1) &\leq t_i = \sum\limits_{j=1}^{i-1} \left( w_j + z_j \right)
\end{array}
\end{equation*}
%
Now, for \useful cycles, we can apply Lemma~\ref{lem:helpfulZi} on the right side and Lemma \ref{lem:axioms} ii) on the left side and solve for $\beta$:
\begin{equation}
\label{eq:worst-cycle-beta}
\beta \leq \frac{\nicefrac{3}{2}- \varepsilon}{1 - 2 \varepsilon}
\end{equation}
%
So for all \useful cycles the ratio within the cycle does not exceed $1 + \beta \varepsilon$, i.e.
\begin{equation*}
\frac{W_i^\mu}{w_i + z_i} \leq 1 + \beta \varepsilon
\quad \Leftrightarrow \quad
W_i^\mu \leq (1+\beta \varepsilon)(w_i + z_i)
\end{equation*}
%
Applying Lemma \ref{lem:axioms} i) to the left and subsequently Lemma \ref{lem:axioms} ii) to the right side results in 
%\begin{equation}
%\label{eq:beta}
$z_i + z_{i+1} \leq z_i + \beta\varepsilon z_i + (1+\beta\varepsilon w_i)$, which in turn gives the following lemma.
%\end{equation}
\begin{lemma}
\label{lem:helpfulCycles}
In helpful cycles, we have
\begin{equation*}
z_{i+1} \leq (1 + 2 \beta)w_i = \left(1 + \frac{3-2\varepsilon}{1-2\varepsilon} \, \varepsilon\right)w_i.
\end{equation*}
\end{lemma}
%
Now consider a $z_{i+1}$ from a \useful cycle as depicted in \autoref{fig:low-bound-cycle}.
\begin{figure}[ht]
	\centering
	\includegraphics[width=.9\textwidth]{figures/low-bound-cycle}
	\caption{A depiction of interweaving of the directional \ratio of left and right $i$-cycles}
	\label{fig:low-bound-cycle}
\end{figure}
%
By Lemma~\ref{lem:helpfulCycles}, we can bound $z_{i+1}$ in terms of $w_i$.
In turn, we want to bound $w_{i}$ in terms of $y_{h+1}$.
As established in the proof of Lemma~\ref{lem:rl-interval}, the cycle endpoint at $t_{i+1}$ with it consumption $\geq 1$ must lie within $r_{h+1}$ to the right of the minimum at $t_{h}+y_{h+1}$ to keep to total \ratio below $(\nf{3}{2} + \varepsilon)$.
Equivalently, the minimum at $t_{i} + z_i$ can only lie $r_{i}$ to the left of $t_{h+1}$, as seen in \autoref{fig:low-bound-cycle}. Hence
\begin{equation*}
w_i \leq y_{h+1} + r_i + r_{h+1}\\
\end{equation*}
%
Applying Lemma~\ref{lem:rl-interval} results in
\begin{equation*}
w_i \leq y_{h+1} + \frac{\varepsilon}{\nicefrac{1}{2} - \varepsilon} (t_i + z_i) + \frac{\varepsilon}{\nicefrac{1}{2} - \varepsilon} (t_{h+1} + y_{h+1}).
\end{equation*}
%
Note, that the $r_i$ is only relevant if $t_i + z_i \leq t_{h+1}$, so we can assume as much.
Then applying Lemma~\ref{lem:helpfulZi} and Lemma~\ref{lem:rl-interval} we obtain
\begin{equation}
\label{ineq:step-2}
\def\arraystretch{2}
\begin{array}{ r l }
w_i &\leq y_{h+1} + \frac{\varepsilon}{\nicefrac{1}{2} - \varepsilon} (t_{h+1}) + \frac{\varepsilon}{\nicefrac{1}{2} - \varepsilon} (t_{h+1} + y_{h+1}) \\
&\leq y_{j+1}\left(1 + \frac{\varepsilon}{\left(\nicefrac{1}{2} - \varepsilon\right)^2} + \frac{\varepsilon \left(\nicefrac{1}{2} + \varepsilon\right)}{\left(\nicefrac{1}{2} - \varepsilon\right)^2}\right).
\end{array}
\end{equation} 
%
Lemma~\ref{lem:helpfulCycles} and Lemma~\ref{lem:rl-interval} can be applied to derive equivalent bounds for $y_{h+1}$, in terms of $v_j$ and $v_j$ in terms of $z_i$:
\begin{equation}
\label{ineq:step-3}
y_{h+1} \leq \left(1 + \frac{3-2\varepsilon}{1-2\varepsilon} \, \varepsilon\right)v_j
\quad\text{ and }\quad
v_{j} \leq z_{i}\left(1 + \frac{\varepsilon}{\left(\nicefrac{1}{2} - \varepsilon\right)^2} + \frac{\varepsilon \left(\nicefrac{1}{2} + \varepsilon\right)}{\left(\nicefrac{1}{2} - \varepsilon\right)^2}\right).
\end{equation}
%
Combining all arguments from Lemma~\ref{lem:helpfulCycles}, Inequality \ref{ineq:step-2} and Inequality \ref{ineq:step-3} to bound $z_{i+1}$ directly in terms of $z_i$ and $\varepsilon$ yields
\begin{equation}
\label{ineq:2}
z_{i+1} \leq \left(1 + \frac{3-2\varepsilon}{1-2\varepsilon} \, \varepsilon\right)^2 \left(1 + \frac{\varepsilon}{\left(\nicefrac{1}{2} - \varepsilon\right)^2} + \frac{\varepsilon \left(\nicefrac{1}{2} + \varepsilon\right)}{\left(\nicefrac{1}{2} - \varepsilon\right)^2}\right)^2 z_i.
\end{equation}
%
On the other hand, Lemma~\ref{lem:helpfulZi} gives a bound in the other direction:
\begin{equation}
\label{ineq:3}
z_{i+1} \geq \frac{\nicefrac{1}{2}- \varepsilon}{\nicefrac{1}{2} + \varepsilon} \sum\limits_{j=1}^{i} \left( w_j + z_j \right) \geq \frac{\nicefrac{\textsl{}1}{2}- \varepsilon}{\nicefrac{1}{2} + \varepsilon} (w_i + z_i) \geq \frac{1- 2 \varepsilon}{\nicefrac{1}{2} + \varepsilon} \, z_i.
\end{equation}
%
Satisfying both Inequality \ref{ineq:2} and Inequality \ref{ineq:3} yields a contradiction unless $\varepsilon \geq 0.03069$, which gives the following lower bound.
\begin{theorem}
There exist no \crews for a speed $v< 1.53069$. %, which is a non-trivial improvement over the $\nicefrac{3}{2}$-bound.
\end{theorem}
%
Note that this exact bound assumes that \useful cycles are consecutive.
However, if this is not the case, one can achieve an even stronger bound by similar technique. %using among mostly identical estimations and the fact that $w_i$ then lies completely within an $l_{k+1} + r_{k+1}$-sized interval around $t_{k+1} + z_{k+1}$. % the interval $[t_{k+1} + z_{k+1} - l_{k+1}, t_{k+1} + z_{k+1} + r_{k+1}]$.
%
%It stands to reason that there might be some additional improvements possible by tightening the inequalities.


==> includes/lowerBound_BothLeft.tex <==
\section{A lower bound of $v>1.5$}
First, we show that not all possible \crewss have to be considered.

\begin{lemma}[Increasing \wall lengths]
	\label{lem:increasing-walls}
	For any \crews $\mathcal{S}$ viable for a speed $v$, there exists a \crews consisting of vertical \walls of strictly increasing length in each direction which is also viable for $v$.	
	That is, $\B_{i +1} > \B_i$ and $\D_{i+1} > \D_i$, $\forall i$.
\end{lemma}

\begin{proof}
	Assume $\mathcal{S}$ contains a vertical \wall $w_2$ that is at most as long as the previous one $w_1$ in that direction.
	Then consider the \crews $\mathcal{S}' = \mathcal{S} \setminus {w_2}$.
	Removing $w_2$ does not decrease the shortest $L_1$ path from the \fire origin $(0,0)$ to any point in the plane including points on all other \walls, as those paths are prolonged by $w_1$.
	However, $w_2$ is no longer consumed and hence the total \burn $\BF{\mathcal{S'}}(t) \leq \BF{\mathcal{S}}(t)$ for all $t$ and therefore $\QF{\mathcal{S}'}(t) \leq \QF{\mathcal{S}}(t)$.
\end{proof}

\begin{theorem}[Lower Bound]
	\label{thm:lowerbound}
	There exists no \crews which is viable for speeds $v<1.5$.
\end{theorem}

\begin{proof}
The idea of the proof is to show that the ratios \consumptionRatio[l,r] are always larger than $0.5$, for $t$ greater than some threshold and sometimes exceed $1$ for arbitrarily large $t$.
We start with the latter.

Assume there exists a \crews $\mathcal{S}^{*}$ which is viable for $v<1.5$.
For every time $t_0 > 0$ there must exist some point in time $t_1 > t_0$, where the current \burn is at most $ 1$.
Because the current consumption takes on integer values, it would otherwise be greater or equal than $2$ all the time, requiring speed $v\geq 2$.
Hence, at $t_1$ at least for one of the directions the current \burn is $0$.
This can only happen if the fire burns along the back of a vertical \wall and has fully consumed all \walls previously touched in this direction.
For example, such a $0$-interval can be seen at $d_2$ in \autoref{fig:baseExample}.

\Wlog assume this happens on the left-hand side.
By Lemma~\ref{lem:increasing-walls}, we can also assume that \walls are strictly increasing in length in both directions.
Consider the time $t$ and total \burn $\BF{\mathcal{S}^{*}}^l(t)$ in the left direction at the beginning of a $0$-interval.
For an explanation of the $\max(0, 2 \B_{i-1} - \B_i)$ summand, see \autoref{fig:0-interval-start}.
\begin{figure}[ht]
	\centering
	\includegraphics[height=3cm,page=1]{figures/0-interval-beginning}
	\caption{
		The two possible configurations at the beginning of a $0$-interval at time $t$. 
		In the first case, the \fire reached the lower end of the $\B_{i}$ \wall first, so the $0$-interval starts exactly when the upper end is reached.
		In the second case, the upper end was reached first, so the $0$-interval begins when the lower end is reached after additional time $2 \B_{i-1} - \B_i$.
	}
	\label{fig:0-interval-start}
\end{figure}
\begin{center}
	$t 	 =   \sum\limits_{k=1}^i \A_k + \B_i + \max(0, 2 \B_{i-1} - \B_i)$ \quad\quad\quad
	$\BF{\mathcal{S}^{*}}^l(t)  =  \sum\limits_{k=1}^i \A_k + \sum\limits_{k=1}^i \B_k -  \startWall$
\end{center}

Assume \,$\QF{\mathcal{S}^{*}}^l(t) \leq 1$, then $\frac{\BF{\mathcal{S}^{*}}^l(t)}{t} \leq 1$ and $\BF{\mathcal{S}^{*}}^l(t) \leq t$
\begin{equation*}
\def\arraystretch{2}
\begin{array}{l r c l }
\Rightarrow 	
	& \sum\limits_{k=1}^i \A_k + \sum\limits_{k=1}^i \B_k - \startWall 
	&\leq 
	& \sum\limits_{k=1}^i \A_k + \B_i + \max(0, 2 \B_{i-1} - \B_i) \\
	%\Leftrightarrow \sum\limits_{k=1}^i \B_k  &> \B_i + \max(0, 2 \B_{i-1} - \B_i) + \startWall \\
\Rightarrow 
	& \sum\limits_{k=1}^{i-2} \B_k + \B_{i-1} + \B_{i}
	& \leq
	& \max( \B_i, 2 \B_{i-1}) + \startWall
\end{array}
\end{equation*}
Due to Lemma~\ref{lem:increasing-walls} $\B_{i-1} + \B_{i} > \max(\B_i, 2 \B_{i-1})$ and $\sum_{k=1}^{i-2} \B_k > (i-2) \cdot \B_1 > \startWall$ for $i$ larger than some threshold $i_0$.
As the left-hand current \burn is $0$ for arbitrarily large $t$, we can assume $i>i_0$.
But this is a contradiction.
Hence $\QF{\mathcal{S}^{*}}^l(t) > 1$ at the beginnings of all $0$-intervals after some threshold $t_0$ in the left-hand direction.

Hence for the whole \crews $\mathcal{S}^{*}$ to be viable for $v<1.5$, the \ratio $\QF{\mathcal{S}^{*}}^r(t)$ in the right-hand direction must be below $0.5$ at exactly these moments.
Hence for the right-hand direction $0$-intervals exist for arbitrarily large $t$.

The ends of those $0$-intervals are local minima of that directions \ratio.
Consider the time $t$ and total \burn $\BF{\mathcal{S}^{*}}^r(t)$ in the right-hand direction at the end of such an interval.
For an explanation of the $\min(\A_{i+1}, \B_i)$ summand, see \autoref{fig:0-interval-end}.
\begin{figure}[ht]
	\centering
	\includegraphics[height=3cm,page=1]{figures/0-interval-end}
	\caption{
		The two possible configurations at the end of a $0$-interval at time $t$. 
		In the first case, the $0$-interval ends, when the \fire reaches the highway, $\B_i$ time units after passing the top of the $\B_i$ \wall.
		In the second case, the next \wall is reached before the highway, so the $0$-interval ends, $\A_{i+1}$ time units after passing the top of the $\B_i$ \wall.
	}
	\label{fig:0-interval-end}
\end{figure}

\begin{center}
	$ t = \sum\limits_{k=1}^i \A_k + \B_i + \min(\A_{i+1}, \B_i) $ \quad\quad\quad $\BF{\mathcal{S}^{*}}^r(t) = \sum\limits_{k=1}^i \A_k + \sum\limits_{k=1}^i \B_k - \startWall$
\end{center}
Assume $\QF{\mathcal{S}^{*}}^r(t) < 0.5$, then $\frac{\BF{\mathcal{S}^{*}}^r(t)}{t} < 0.5$ and $2 \cdot \BF{\mathcal{S}^{*}}^r(t) < t$
\begin{equation*}
\begin{array}{l r c l}
\Rightarrow
	& 2 \cdot \sum\limits_{k=1}^i \A_k + 2 \cdot \sum\limits_{k=1}^i \B_k - 2 \startWall
	& <
	& \sum\limits_{k=1}^i \A_k + \B_i + \min(\A_{i+1}, \B_i) \\
\Rightarrow
	& \sum\limits_{k=1}^i \A_k + 2 \cdot \sum\limits_{k=1}^i \B_k  
	& <
	& 2 \B_i  + 2 \startWall
\Rightarrow \sum\limits_{k=1}^i \A_k + 2 \cdot \sum\limits_{k=1}^{i-1} \B_k < 2 \startWall
\end{array}
\end{equation*}

As above $\sum_{k=1}^{i-1} \B_k > (i-1) \B_1 > 2 \startWall$ for $i$ larger than some threshold $i_0$.
Hence after some threshold time $t_0$, even at the local minima the \ratio of the right-hand direction is above $0.5$, hence it is always above $0.5$.
Therefore $\QF{\mathcal{S}^{*}}(t)$ exceeds $1.5$ for arbitrarily large $t$, which makes $\mathcal{S}^*$ not viable for $v<1.5$.
\end{proof}


==> includes/model.tex <==
\section{Model}
\label{section:modelDefinition}
In our model, the \fire originates from the origin and continuously expands over time with speed $1$ according to the $L_1$ metric.
To prevent the fire from immediately spreading into the lower half-plane, we allow an arbitrarily small head-start of barrier of length $\startWall$ into both directions along the $x$-axis.

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.75\textwidth]{figures/SpreadingFire}
	\caption{Fire spreading along delaying barriers}
	\label{fig:delayingBarriers}
\end{figure}
Assume that a system of \walls has been built.
The \crews consists of a horizontal \wall containing the fire in the upper half-plane and several vertical delaying barriers attached to it.
As the fire spreads over the \crews, it represents a geodesic $L_1$ circle, which consumes the \walls when burning along them.
We consider a piece of the \wall as {\em consumed} as soon as the \fire has reached this piece for the first time.
The effect of delaying \walls is illustrated in \autoref{fig:delayingBarriers}.
As one can see, when the fire reaches a delaying barrier for the first time, it may burn along \walls at multiple points.
However, after passing the top of a \wall there is no \burn for a while as the delaying \wall has already been burned along from the other side.
We call the number of such \burn points the {\em current \burn} and an interval with $k$ \burn points a {\em $k$-interval}. 
However, while the current \burn is always an integer value, it may vary depending mainly on the exact placement and lengths of delaying barriers.
Therefore, we define the \emph{total \burn} $\BF{}$ and \emph{\ratio} $\QF{}$ for a time interval $\left[t_1, t_2\right]$ in a \crews:
\begin{equation*}
\begin{array}{r l}
\BF{}(t_1, t_2) 
	& := \text{length of all pieces of \walls consumed by the fire between } t_1 \text{ and } t_2\\
\QF{}(t_1, t_2) 
	& := \frac{ \BF{}(t_1, t_2)}{t_2 - t_1}\,.
\end{array}
\end{equation*}
For the \burn in a time interval $[0, t]$, we will also write $\BF{}(t)$ for short.
Note that all these definitions can easily be applied to either side of the \crews, denoted by \consumptionRatio[l] and \consumptionRatio[r].
Obviously, $\consumptionRatio = \consumptionRatio[l] + \consumptionRatio[r]$.

For a limited speed $v$, it is necessary and sufficient to have $\BF{}(t) \leq v \cdot t$ for all times $t$, which means $v \geq \sup_t \QF{}(t)$.
The question then obviously is: What is the minimum speed $v$ for which such a \crews exists?


==> includes/recursiveStrategy.tex <==
\section{A viable \crews for {$v = 1.8944 \dots$}}
Assume we want to construct a \crews $\mathcal{S}$ improving on the naive strategy, which is viable for $v=2$.
The \ratio only decreases when the current \burn is below the current ratio.
As the current \burn is an integer value, this only happens when it is at most $1$, which means we have a $0$-interval in at least one direction.
Hence we would want these intervals to be as long as possible, which results in the following conditions:
\begin{align*}
\A_{i+1} &\geq \B_{i} \,\,\, \wedge \,\,\, \B_{i+1} \geq 2 \B_{i}  &\forall i \geq 1 \\
\text{equivalently } \C_{i+1} &\geq \D_{i} \,\,\, \wedge \,\,\, \D_{i+1} \geq 2 \D_{i}  &\forall i \geq 1
\end{align*}
This forces the $0$-intervals to always start exactly when the \fire reaches the upper end of a vertical wall and end when the \fire reaches the \highway again after burning along 
the full length along the back of the already consumed vertical wall; see \autoref{fig:0-interval-start} and \ref{fig:0-interval-end}.
For a single direction this results in a repeating cycle of time intervals as seen in \autoref{fig:interval-cycle}.
%
\begin{figure}[ht]
	\centering
	\includegraphics[width=\textwidth]{figures/IntervalCycleWithIllustration}
	\caption{A repeating time interval cycle. The values $0, 1$ and $3$ denote the current \burn in this direction.}
	\label{fig:interval-cycle}
\end{figure}
%
From our reasoning about the lower bound, we know that $0$-intervals are necessary for both directions in order to achieve $v<2$.
%But we also know by a similar argument as in the proof of Theorem \ref{thm:lowerbound}, that we must repeatedly have $0$-\burn intervals in both directions and that both direction on their own will have a a \ratio $\geq 1$ at the beginning of these intervals.
The idea is to construct the \crews in such a way that the $0$-intervals always appear in an alternating fashion, so the local maxima in the \ratio of one direction can be countered by the $0$-intervals of the other direction.

Consider the periodic interlacing of time intervals as illustrated in \autoref{fig:recursiveInterlacing}, where the end point of the $0$-interval from one direction coincides with the beginning of the \mbox{$3$-interval} of the other direction.
\begin{figure}[ht]
	\centering
	\includegraphics[width=.9\textwidth]{figures/RecursiveIntervals}
	\caption{The periodic interlacing of time intervals.}
	\label{fig:recursiveInterlacing}
\end{figure}

%Assume the combined \ratio of both direction at $t_1$ is $\mu$ for some $\mu \in (1,2)$.
The current \burn is always greater than $1$, since the $0$-intervals do not overlap.
As we are trying to construct a \crews viable for some $v<2$, $\QF{\mathcal{S}}(t)$ must be smaller than $2$ at all times.
Then, $t_1$, $t_3$ and $t_5$ have to be local maxima, while $t_2$, $t_4$ and $t_6$ have to be local minima of $\QF{\mathcal{S}}(t)$. 
The idea to ensure that the global maximum of $\QF{\mathcal{S}}(t)$ stays below $2$ is to make all local maxima attain the same value $\mu$ and hope that it stays below~$2$.

So let $\mu := \QF{\mathcal{S}}(t_1)$.
Then $\QF{\mathcal{S}}(t_3) = \mu$ if and only if, between $t_1$ and $t_3$, the ratio of consumption over time interval length is also $\mu$.
Thus,
%\begin{align*}
%\QF{\mathcal{S}'}(t_3) &= \frac{\BF{\mathcal{S}'}(t_3)}{t_3}\\
%&= \frac{\BF{\mathcal{S}'}(t_1) + (\BF{\mathcal{S}'}(t_3)-\BF{\mathcal{S}'}(t_1))}{t_1 +  (t_3-t_1)} \\
%&= \frac{t_1}{t_3} \frac{\BF{\mathcal{S}'}(t_1)}{t_1} + \frac{t_3-t_1}{t_3} \frac{\BF{\mathcal{S}'}(t_3)-\BF{\mathcal{S}'}(t_1)}{t_3-t_1} \\
%&= \frac{t_1}{t_3} \QF{\mathcal{S}'}(t_1) + \frac{t_3-t_1}{t_3} \frac{\BF{\mathcal{S}'}(t_3)-\BF{\mathcal{S}'}(t_1)}{t_3-t_1} \\
%&= \frac{t_1}{t_3} \mu + \frac{\BF{\mathcal{S}'}(t_3)-\BF{\mathcal{S}'}(t_1)}{t_3-t_1}
%\end{align*}
\begin{equation*}
\def\arraystretch{1.4}
\begin{array}{l r l}
					& \frac{\B_i \cdot (0 + 1) + \D_{i-1} \cdot (1 + 3) + (\D_{i}-2\D_{i-1}) \cdot (1+1)}{\B_i + \D_{i-1} + \D_{i}-2\D_{i-1}} &= \mu \\
\Leftrightarrow	& \B_i + 2\D_i &= \mu (\B_i + \D_i - \D_{i-1})\\
\Leftrightarrow	& \D_i &= \frac{\mu - 1}{2 - \mu}\B_i - \frac{\mu}{2-\mu} \D_{i-1}\,.
\end{array}
\end{equation*}
%
%Hence, if we can then choose $\A_i$, $\B_i$, $\C_i$ and $D_i$ such that $QF{\mathcal{S}'}(t_1) = QF{\mathcal{S}'}(t_3) = QF{\mathcal{S}'}(t_5)$, as well as construct a suitable starting situation, this defines a \crews viable for $v<2$.
%
%Assume we knew the combined \ratio at $t_3$ lies somewhere in the interval $(1,2)$, so $1 < \QF{\mathcal{S}'}(t_3) < 2$.
%Then we know that $t_3$ is a local maximum of the \ratio, as the total \burn before $t_3$ was $2$, so $\QF{\mathcal{S}'}$ was increasing, but is $1$ after $t_3$, so $\QF{\mathcal{S}'}$ will be decreasing.
%Then we know $QF{\mathcal{S}'}(t_2) < \QF{\mathcal{S}'}(t_3)$ as the total current \burn between $t_2$ and $t_3$ is always $\geq 2$.
%
Similarly, by applying the same reasoning to $t_3$ and $t_5$, we obtain a second recursive formula $\B_{i+1} = \frac{\mu - 1}{2 - \mu}\D_i - \frac{\mu}{2-\mu} \B_{i}$.
Together these recursions can be represented by a matrix and solved by applying standard techniques.
The values for $\A_i$ (and $\C_i$) can be expressed as linear combinations of $\D_i$ and $\B_i$ -- see the interval between $t_2$ and $t_4$ ($t_4$ and $t_6$) in \autoref{fig:recursiveInterlacing}.

Analysing the zeros of the characteristic polynomial indicates that this recursion has real solutions for $b_i$ and $d_i$ as long as $\mu \geq (2 +\sqrt{5})/{\sqrt{5}}$.
For the limiting case $\mu = (2 +\sqrt{5})/{\sqrt{5}} = 1.8944 \dots $, we get $\B_i = \left(2+\sqrt{5}\right) \D_{i-1} =  \left(2+\sqrt{5}\right)^2 \B_{i-1}$.

To prove the final theorem, it remains to find initial values to get the recursion started, while maintaining $\QF{\mathcal{S}}(t) \leq \mu$.
Suitable values are
\begin{equation*}
\begin{array}{r l  r l  r l }
\B_i & := \startWall \cdot \left(2 + \sqrt{5}\right)^{2i}
	& \hspace*{1cm}\mu  	&:= \frac{2 +\sqrt{5}}{\sqrt{5}} \approx 1.8944
	& \hspace{1cm}\C_1 &:= \frac{\left(\mu-2 \right) \D_1 + 2 \startWall + \B_1}{2 - \mu}\\
\D_i & := \startWall \cdot \left(2 + \sqrt{5}\right)^{2i+1}
	& \A_1	&:= \startWall
	& \A_2 &:= 2\D_1 + \C_1 - \A_1 - \B_1,\\
\end{array}
\end{equation*}
which results in intervals given in \autoref{fig:intervalStart}.
Note that all barrier lengths only depend \mbox{on $s$.} 
%\begin{figure}[ht]
%	\centering
%	\includegraphics[width=\textwidth, page= 3]{figures/StartWalls}
%	\caption{Starting situation}
%	\label{fig:startWalls}
%\end{figure}
\begin{figure}[ht]
	\centering
	\includegraphics[width=.8\textwidth]{figures/StartIntervals}
	\caption{Illustration of time intervals for a suitable starting situation.}
	\label{fig:intervalStart}
\end{figure}
%
%As $\QF{\mathcal{S}_\mu}(t) = 0$ for any $t<\startWall$, it is clear, that $t_{s1}$, $t_{s2}$ and $t_{s4}$ are the local maxima.
%%Additionally for the starting situation to properly transition into the recursive one, the end of the $0$-intervals for $\D_1$ and $\B_2$ must actually coincide with the beginning of the $3$-intervals for $\B_1$ and $\D_1$.
%Additionally, if the interval ends actually coincide in $t_{s3}$ and $t_{s5}$, then $t_{s3}$, $t_{s4}$ and $t_{s5}$ are equivalent to $t_3$, $t_4$ and $t_5$ for $i=1$ as in the recursive situation, which gives a proper transition.
%It remains to choose $\B_1, \C_1, \D_1, and \A_2$ such that $\QF{t_1}$, $\QF{t_2}$ and $\QF{t_3}$ are all $\leq \mu$ and the intervals properly coincide in $t_{s3}$ and $t_{s5}$.
%
%\begin{align*}
%\R &:= \left(2 + \sqrt{5}\right) \approx 4.23 \\
%\mu &:= \frac{2+\sqrt{5}}{\sqrt{5}}\\
%\B_i &:= \startWall \cdot \R^{2i} \\
%\D_i &:= \startWall \cdot \R^{2i+1}\\
%\A_1 &:= \frac{\left(\mu - 2 \right) \B_1 + 2 \startWall}{2-\mu} = \startWall \\
%\C_1 &:= \frac{\left(\mu-2 \right) \D_1 + 2 \startWall + \B_1}{2 - \mu} =
%\startWall \cdot \left(\R^2 + 2 \frac{\sqrt{5}}{\sqrt{5}-2} + \frac{ \sqrt{5}}{\sqrt{5}-2} \R^3 \right) \approx 113 \cdot \startWall\\
%\A_2 &:= 2\D_1 + \C_1 - \A_1 - \B_1 = \startWall \left( 2\R^{3} + \R^2 + 2 \frac{ \sqrt{5}}{\sqrt{5}-2} + \frac{ \sqrt{5}}{\sqrt{5}-2} \R^3 \right) - 1 - \R^{2} \approx 246 \cdot \startWall\\
%%\A_i &:= 2\D_{i-1} + \B_{i-1} - \D_{i-2} = 2\R^{2i-1} - \R^{2i-2} - \R^{2i-3}\\
%%\C_i &:= 2\B_i + \D_{i-1} - \B_{i-1} = 2\R^{2i} - \R^{2i-1} - \R^{2i-2}
%\end{align*}
%
%The only variable determining $\QF{\mathcal{S}_\mu}(t_{s1})$ is $\B_1$,
%as $\QF{t_{s1}} = \frac{2 \B_1}{\B_1 + \startWall}$. Choosing $\B_1$ such that $\QF{t_{s1}} = \mu$ results in $\B_1 = \startWall \cdot \left(2 + \sqrt{5}\right)^2 \approx 17.89 \startWall $.
%From the recursive formula then follows an explicit formula for all $\B_i$ and $\D_i$:
%\[\B_i = \startWall \cdot \left(2 + \sqrt{5} \right)^{2i} \,\,\, \text{ and } \,\,\, 
%\D_i = \startWall \cdot \left(2 + \sqrt{5} \right)^{2i+1}
%\]
%
%Similarily $\C_1$ is then the only unknown variable determining $\QF{\mathcal{S}_\mu}(t_{s2})$, which results in $\C_1 = \frac{\left(\mu-2 \right) \D_1 + 2 \startWall + \B_1}{2 - \mu} \approx 113 \startWall$ for $\QF{\mathcal{S}_\mu}(t_{s2}) = \mu$.
%%, as $\QF{t_{s2}} = \frac{2 \left(\D_1 + \C_1 - \startWall \right) - \B_1}{\D_1 + \C_1}$,
%$\A_2$ then directly follows from the need of coinciding interval ends in $t_{s3}$ and the already determined wall lengths with $\A_2 := 2\D_1 + \C_1 - \A_1 - \B_1 \approx 246 \startWall$.
%
%All further $\A_i$ and $\C_i$ then follow from the recursion, hence we have constructed a suitable starting situation for the recursion with positive real values for all \wall lengths.
%As such, the recursive interval interlacing together with this starting construction result in a \crews $\mathcal{S}_\mu$, with $\QF{\mathcal{S}_\mu}(t) = \mu$ in repeating local maxima and hence the following theorem holds:
\begin{theorem}
The highway can be protected with speed $v > \mu = \frac{2 +\sqrt{5}}{\sqrt{5}} =  1.8944 \dots$
\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Following is an incomplete more detailed description of the starting situation, but the shortened version above is probably more suitable for the limited space of EuroCG.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%After reaching the end of the given initial starting wall, the fire by construction reaches the first vertical wall of length $\B_i$ in the left direction as $\A_i = \startWall$.
%It will then burn along it with a current \burn of $1$ in the left direction and along the \highway with a current \burn of $1$ in the right direction for an overall current \burn of $2$.
%As $\C_1 > \A_1 + \B_1$, the fire will reach the end of the first vertical wall in the left direction before reaching the first wall in the other direction, $\QF{\mathcal{S}_\mu}$ reaches it first local maximum at $t_1 = \A_1 + \B_1$.

%\begin{align*}
%	\QF{\mathcal{S}_\mu}(t_1) &= \frac{2 \cdot \left( \A_1 + \B_1 - \startWall \right)}{\A_1 + \B_1} \\
%	&= \frac{2 \left( \frac{\left(\mu - 2 \right) \B_1 + 2 \startWall}{2-\mu} + \B_1 - \startWall \right)}{\frac{\left(\mu - 2 \right) \B_1 + 2 \startWall}{ 2 - \mu} + \B_1} \\
%	&= \frac{2 \left( \left(\mu - 2 \right) \B_1 + 2 \startWall + \left( 2 - \mu \right)\B_1 - \left( 2 - \mu \right) \startWall \right)}{\left(\mu - 2 \right) \B_1 + 2 \startWall + \left( 2 - \mu \right) \B_1} \\
%	&= \frac{2 \mu s}{2s} = \mu >1 \\
%	%&= \frac{s \cdot \R^{2}}{s + s\R^{2}}\\
%	%&= \frac{ 2 (2 + \sqrt{5})^2}{1 + (2 + \sqrt{5})^2}\\
%	%&= \frac{8 + 8 \sqrt{5} + 10}{1 + 4 + 4 \sqrt{5} + 5}\\
%	%&= \frac{18 + 8 \sqrt{5}}{10 + 4 \sqrt{5}} \\
%	%&= \frac{2 + \sqrt{5}}/{\sqrt{5}} > 1
%\end{align*}
%
%After passing the end of the first wall, the current \burn in the left direction is $0$ until the \fire reaches either the \highway after $\B_1$ time or the next vertical wall in that direction after $\A_2$ time..
%As $\A_2 > \B_1$, the former will happen first.
%The current \burn will then be $1$ until the fire also reaches the vertical wall after $\A_2 - \B_1$ time, at which it will change to $3$ as the fire will burn along the $highway$ as well as both up and down along the second vertical wall until it reaches either end of it.
%As $\B_2 > 2 \B_1$, the fire will reach the lower end touching the \highway first, after which the \burn will change back to $1$ until the fire reaches the upper end of the vertical wall.
%
%
%\begin{figure}[ht]
%	\centering
%	\includegraphics[scale=0.5]{figures/exampleFigure}
%	\caption{Placeholder figure}
%	\label{fig:consumption-interval}
%\end{figure}
%\BS{TODO: Picture \burn intervals at this situations.}
%
%In the right direction the fire will reach the first vertical wall at time $\C_1$ and its upper end at $\C_1 + \D_1$. As $ \A_1 + 2 \B_2 < \C_1 + \D_1 < \A_1 + \A_2 + \B_1$, this will happen after the \fire reaches the highway again after the first vertical wall but before it reaches the second vertical wall in the left direction.
%Hence, $\QF{\mathcal{S}_\mu}$ reaches it second local maximum at $t_2 = \C_1 + \D_1$.
%
%\begin{align*}
%\QF{\mathcal{S}_\mu}(t_2) &= \frac{2 \cdot \left( \C_1 + \D_1 - \startWall \right) - \B_1}{\C_1 + \D_1} \\
%&= \frac{2 \cdot \left( \frac{\left(\mu-2 \right) \D_1 + 2 \startWall + \B_1}{2 - \mu} + \D_1 - \startWall \right) - \B_1}{\frac{\left(\mu-2 \right) \D_1 + 2 \startWall + \B_1}{2 - \mu} + \D_1} \\
%&= \frac{2 \cdot \left( \left(\mu-2 \right) \D_1 + 2 \startWall + \B_1 + \left( 2 - \mu \right) \D_1 - \left( 2 - \mu \right) \startWall \right) - \left( 2 - \mu \right) \B_1}{\left(\mu-2 \right) \D_1 + 2 \startWall + \B_1 + \left( 2 - \mu \right) \D_1} \\
%&= \frac{2 \left( \mu s + \B_1 \right) - \left(2 - \mu \right ) \B_1}{2s + \B_1} = \frac{2 \mu s + \mu s}{2s + \mu} = \mu
%%&= \frac{s \cdot (2\left(\R^2 + 2 \frac{\sqrt{5}}{\sqrt{5}-2} + \frac{ \sqrt{5}}{\sqrt{5}-2} \R^3 \right) + 2\R^{3} - 2}{s + s\R^{2}}\\
%%&= \frac{ 2 (2 + \sqrt{5})^2}{1 + (2 + \sqrt{5})^2}\\
%%&= \frac{8 + 8 \sqrt{5} + 10}{1 + 4 + 4 \sqrt{5} + 5}\\
%%&= \frac{18 + 8 \sqrt{5}}{10 + 4 \sqrt{5}} \\
%%&= \frac{2 + \sqrt{5}}/{\sqrt{5}} > 1
%\end{align*}
%
%By the choice of $\A_2$, the moment when the fire reaches the second vertical wall in the left direction and when it reaches the \highway the first time after passing the first vertical wall in the right direction coincide.
%



==> includes/recursiveStrategyImproved.tex <==
\newcommand{\constOffset}{\ensuremath{\delta}\xspace}
\subsection{Improving the upper bound}
It is possible to reduce the upper bound of $v=1.\overline{8}$ slightly.
As shown in \autoref{fig:recursiveInterlacing}, the end of the $3$-interval in one direction coincided with the end of the $0$-interval in the other direction, which made $t_4$ the only local maximum of the interval $[t_1, t_4]$.
We introduce a regular shift by a factor of \constOffset , see \autoref{fig:recursiveInterlacingImproved}.
This allows the $3$-interval in one direction to lie completely inside the $0$-interval of the other direction, as shown in \autoref{fig:recursiveInterlacingImproved}.
Then, there are two local maxima in the equivalent interval $[t_1, t_5]$, namely at $t_3$ and $t_5$.
We force both maxima to attain the same value to minimize both at the same time.

%Note that the interlacing of time intervals in \autoref{fig:recursiveInterlacing} is a special case of the periodic interlacing of time intervals illustrated in \autoref{fig:recursiveInterlacingImproved}.
\begin{figure}[ht]
	\centering
	\includegraphics[width=\textwidth]{figures/RecursiveIntervalsImproved}
	\caption{A general periodic interlacing of time intervals.}
	\label{fig:recursiveInterlacingImproved}
\end{figure}
Again, we set $d_i = \constGrowth \cdot b_i$ and $b_{i+1} = \constGrowth \cdot d_i$, for some $\constGrowth \geq 1$ determined below.
Then the value of the first local maximum can be expressed as
\begin{equation*}
\QF{\mathcal{S}}(t_1, t_3) 
	= \frac{\BF{\mathcal{S}}(t_1, t_3)}{t_3 - t_1}
	= \frac{1 \cdot (\constOffset \cdot b_i) + 3 \cdot b_i}{\constOffset \cdot b_i + b_i} 
	= \frac{\constOffset + 3}{\constOffset + 1} 
	= 1 + \frac{2}{\constOffset + 1}.
\end{equation*}
Considering the cycle from $t_1$ to $t_5$ in \autoref{fig:recursiveInterlacingImproved}, we can conclude that $c_{i+1} = b_{i+1} - b_i + \constOffset b_i + \constOffset d_i$.
Similarly, we can proceed on the interval from $t_5$ to $t_8$ to express $a_{i+1}$ in terms of \constGrowth, \constOffset and $b_i$.

Using these identities, we obtain for the second local maximum
\begin{equation*}
\def\arraystretch{1.4}
\begin{array}{rl}
\QF{\mathcal{S}}(t_1, t_5) 
	& = \frac{\BF{\mathcal{S}}(t_1, t_5)}{t_5 - t_1}
		= \frac{1 \cdot (\constOffset \cdot b_i) + 3b_i + 1\cdot (b_{i+1} - 2 b_i ) + 1 \cdot (c_{i+1} - d_i - \constOffset \cdot d_i)}{d_i + (c_{i+1} - d_i) - \constOffset \cdot d_i}\\
	& = \frac{c_{i+1} - \constOffset \cdot d_i}{c_{i+1} - \constOffset \cdot d_i} + \frac{b_{i+1} + \constOffset \cdot b_i + b_i - d_i}{c_{i+1} - \constOffset \cdot d_i}
	  = 1 + \frac{b_{i+1} - b_i + \constOffset \cdot b_i + 2b_i - d_i}{b_{i+1} - b_i + \constOffset b_i}\\
	& = 2 + \frac{2 b_i - d_i}{b_{i+1} - b_i + \constOffset b_i} = 2 + \frac{2 - \constGrowth}{\constGrowth^2 - 1 + \constOffset}.
\end{array}
\end{equation*}
%
As mentioned above, we set both local maxima to be equal, solve for \constOffset and obtain
\begin{equation*}
\delta = \frac{1}{2} \left( \constGrowth - \constGrowth^2 + \sqrt{-12 + 4 \constGrowth + 5 \constGrowth^2 - 2 \constGrowth^3 + \constGrowth^4}\right).
\end{equation*}
Plugging this into either one of the two local maxima and minimizing the resulting function for $\constGrowth\geq 1$, we obtain
\begin{equation*}
\constGrowth = \frac{3}{2} + \frac{1}{6} \left( 513 - 114 \sqrt{6} \right)^{\nf{1}{3}} + \frac{\left( 19 (9 + 2 \sqrt{6}) \right)^{\nf{1}{3}}}{2 \cdot 3^{\nf{2}{3}}} \approx 4.06887 %4.06886470
\end{equation*}
for the optimal value of \constGrowth, $\constOffset \approx 1.2802$ and
\begin{equation*}
v = \frac{1}{6} \left( 10 - \frac{19^{\nf{2}{3}}}{\sqrt[3]{2 (4 + 3 \sqrt{6})}} + \frac{\sqrt[3]{19 (4 + 3 \sqrt{6}))}}{2^{\nf{2}{3}}} \right) \approx 1.8771 %1.877115599
\end{equation*}
as the minimum speed.

Note that the optimal value for \constGrowth satisfies our conditions given in \autoref{equation:conditionsOfRecursion}, so that the \crews can in fact be realized.
Finally, we give suitable values to get the interlacing started:
\begin{equation*}
\begin{array}{r l  r l}
\B_1  		&:= (\constGrowth^2 + (\constGrowth + 1) \constOffset - 1)^{-1}
	& \A_1 & := \C_1 := \startWall := \frac{2-v}{v} \cdot \B_1\\[1em]
\A_{i+1} &:= \constGrowth^{2(i-1)-1}
	& \hspace{1cm}\B_{i+1} &:= \constGrowth^{2i} \cdot \B_{1}\\
\C_{i+1} &:= \constGrowth^{2(i-1)}
	& \D_{i+1} &:= \constGrowth^{2i+1} \cdot \B_1.
\end{array}
\end{equation*}
To keep the expression simple, we fixed a (positive!) value of $\startWall$ as listed above.
%Please note that we fixed the value of \startWall for simplicity.
These values can be rescaled to work for any given \startWall.
\begin{theorem}
The fire can be contained in the upper half-plane with speed $v > 1.8772$.
\end{theorem}


==> includes/recursiveStrategySangSub.tex <==
\section{Upper bounds}
\label{section:upperBounds}
We prove the upper bound by defining a \crews with bounded \ratio.
To describe it, we denote the $i$-th delaying barrier to the right by $b_i$.
The part of the horizontal barrier between $b_{i-i}$ and $b_i$ is denoted by $a_{i}$.
For simplicity, we also refer to their length by $a_i$ and $b_i$.
For the other direction, we use $c_i$ and $d_i$ respectively.

Before we present the construction, we give some intuition.
Assume we want to construct a \crews for $v<2$.
From our reasoning about the lower bound, we know that this requires $0$-intervals in both directions.
Hence we would want these intervals to be as long as possible, which results in the following conditions:
\begin{equation}
\label{equation:conditionsOfRecursion}
\begin{array}{r c c c l}
		& \A_{i+1} \geq \B_{i} 	& \text{and} 	& \B_{i+1} \geq 2 \B_{i}  	&	\forall i \geq 1, \\
\text{similarly } 
		& \C_{i+1} \geq \D_{i} 	& \text{and}	& \D_{i+1} \geq 2 \D_{i}  &	\forall i \geq 1.
\end{array}
\end{equation}
This forces the $0$-intervals generated by $b_i$ to be of length of $b_i$.
%always start exactly when the \fire reaches the upper end of a vertical wall and end when the \fire reaches the \highway again after burning along 
%the full length along the back of the already consumed vertical wall; 
%see \autoref{fig:delayingBarriers} and \ref{fig:0-interval-end}.
For a single direction this results in a repeating sequence of $k$-intervals of specific lengths and $k$ as shown in \autoref{fig:interval-cycle}.
%
\begin{figure}[ht]
	\centering
	\includegraphics[width=\textwidth]{figures/IntervalCycleWithIllustration}
	\caption{
	A sequence of $k$-intervals to the right of $(0,0)$.
	The length is given above each interval and the current \burn below.
%	The values $0, 1$ and $3$ denote the current \burn in this direction.
	}
	\label{fig:interval-cycle}
\end{figure}
%But we also know by a similar argument as in the proof of Theorem \ref{thm:lowerbound}, that we must repeatedly have $0$-\burn intervals in both directions and that both direction on their own will have a a \ratio $\geq 1$ at the beginning of these intervals.
The idea is to construct the \crews in such a way that the $0$-intervals always appear in an alternating fashion, so the local maxima in the \ratio of one direction can be countered by the $0$-intervals of the other direction.

To show that this idea can be realized, we consider the periodic interlacing of time intervals as illustrated in \autoref{fig:recursiveInterlacing}.
There, the ends of the $0$-intervals in one direction coincide with the ends of the \mbox{$3$-intervals} in the other direction that is at $t_3$ and $t_6$.
\begin{figure}[ht]
	\centering
%	\includegraphics[width=.9\textwidth]{figures/kss_interval_1}
	\includegraphics[width=\textwidth]{figures/RecursiveIntervals}
	\caption{The periodic interlacing of time intervals.}
	\label{fig:recursiveInterlacing}
\end{figure}

The current \burn is always greater than $1$, since the $0$-intervals do not overlap.
Also, the combined \ratio $\QF{}(t)$ must be smaller than $2$ at all times.
This also implies that $t_3$ is no local maximum and the \ratio grows towards 2 between $t_3$ and $t_4$.
Hence, by setting $d_i > 2b_i$ we make $t_1$, $t_4$, $t_7$ the local maxima and $t_2$, $t_5$ the local minima of $\QF{}(t)$.

\newcommand{\constShift}{\ensuremath{\alpha}\xspace}
\newcommand{\constGrowth}{\ensuremath{\beta}\xspace}
Let us now consider the \ratio $\QF{}(t_1, t_4)$ of the cycle from $t_1$ to $t_4$.
There are two $1$-intervals involved in this cycle in the right direction.
The first one, where the fire burns along $a_{i+1}$, is of length $a_{i+1}-b_i$ and lies partially in this cycle.
The second one, where the fire crawls up along $b_{i+1}$, is of length $b_{i+1}-2b_i$ and lies completely in this cycle.
%Because vertical barriers $b_i$ and $b_{i+1}$ effects intervals, we cannot set intervals arbitrary except $1$-interval for $a_{i+1}$. This reasion make hard to design a barrier set.
As the beginning of this cycle is given by the start of the $0$-interval on one side and the end is given by the end of the second $1$-interval on the other side, we know that the length of this cycle is $d_i + (b_{i+1} - 2 b_i)$.
The total \burn in this cycle is $1 \cdot d_i + 2 \cdot b_i + 2(b_{i+1} - 2 b_i)$.
Now we define $d_i = \constGrowth\cdot b_{i}$, $b_{i+1} = \constGrowth \cdot d_i$, and $d_i = \constShift + 2b_i$ for some $\constShift, \constGrowth \in \mathbb{R}_{>0}$.
Note that this choice satisfies all our conditions, including $d_i > 2 b_i$, and that $\constShift = (\constGrowth -2)b_i$ and $b_{i+1} = \constGrowth ^2b_i$.
Then the \ratio of the cycle is given by
\begin{equation*}
%\begin{array}{rl}
\QF{}(t_1, t_4) 
	= \frac{\BF{}(t_1, t_4)}{t_4 - t_1}
	= \frac{(\constShift + 2b_i) + 2b_i + 2(b_{i+1}-2b_i)}{(\constShift + 2 b_i) +b_{i+1}-2b_i} 
	= \frac{\constShift + 2b_{i+1}}{\constShift + b_{i+1}}
	= \frac{(\constGrowth-2) + 2\constGrowth^2}{(\constGrowth -2)+ \constGrowth^2}
%\end{array}
\end{equation*}
and attains a minimal value of \nf{17}{9} for $\constGrowth = 4$.
Note that by design, $\QF{}(t_1, t_2)$ and $\QF{}(t_1, t_3)$ stay below \nf{17}{9}, as well.
%We also get $b_{i+1} = 16b_i$ and $a_{i+1} = 7.5 b_i$.
%We repeat this procedure, then the maximum of consumption ratio is $17/9$.
Moreover, if the \ratio has a maximum of \nf{17}{9} at the beginning of the cycle at $t_1$, this will also be the case at the end at $t_4$ as
\begin{equation*}
%\begin{array}{rl}
\QF{}(t_4) 
	= \frac{\BF{}(t_1)+\BF{}(t_1, t_4)}{t_4}
	= \frac{t_1}{t_4} \cdot \frac{\BF{}(t_1)}{t_1} + \frac{t_4 - t_1}{t_4} \cdot \frac{\BF{}(t_1, t_4)}{t_4 - t_1}
%	= \frac{(\constShift + 2b_i) + 2b_i + 2(b_{i+1}-2b_i)}{(\constShift + 2 b_i) +b_{i+1}-2b_i} 
%	= \frac{\constShift + 2b_{i+1}}{\constShift + b_{i+1}}
%	= \frac{(\constGrowth-2) + 2\constGrowth^2}{(\constGrowth -2)+ \constGrowth^2}
	\leq \frac{17}{9}.
%\end{array}
\end{equation*}
Since the cycles change their roles at $t_4$ such that the $0$-interval occurs on the right side of $(0,0)$, the same argument can be used to bound the local \ratio in the following interval and for all subsequent cycles, recursively.
Note that by looking at the time interval from $t_3$ to $t_6$, we can derive a closed form for $c_{i+1}$.
Similarly we proceed for $a_{i+1}$.

To prove the final theorem, it remains to find initial values to get the interlacing started, while maintaining $\QF{}(t) \leq \nf{17}{9}$.
Suitable values are
%\begin{equation*}
%\begin{array}{r l  r l  r l r l}
%\A_1 & :=  0.5 \startWall 
%	& \hspace*{1cm}\B_1  	&:= 0.2 a_{i}
%	& \hspace{1cm}\A_{i+1} &:= 7.5 b_{i}
%	& \hspace{1cm}\B_{i+1} &:= 16 b_{i}\\
%\C_1 & := a_1+1.5b_1
%	& \D_1	&:= 4 b_1
%	& \C_{i+1} &:= 7.5 d_i
%	& \D_{i+1} &:= 16 d_i,\\
%\end{array}
%\end{equation*}
%which results in the starting intervals given in \autoref{fig:intervalStart}.
%Since $t_1$ is the same role with $t_1$ in \autoref{fig:recursiveInterlacing}, we can use the same idea to design intervals after $t_1$. Because $a_1$ and $b_1$ is less than $s$ and $s$ is given, the maximal $\QF{}(t)$ until $t_1$ is less than $\nf{17}{9}$. Note that all barrier lengths only depend \mbox{on $s$.} 
%\begin{figure}[ht]
%	\centering
%	\includegraphics[width=.8\textwidth]{figures/StartIntervals}
%	\caption{Illustration of time intervals for a suitable starting situation.}
%	\label{fig:intervalStart}
%\end{figure}
\begin{equation*}
\begin{array}{r l  r l  r l r l r l}
\A_1 &:= \startWall 
	& \hspace{.5cm}\B_1  	&:= 17 \startWall
	& \hspace{.5cm} \A_2		&:= 34 \startWall
	& \hspace{.5cm}\A_{i+1} &:= 7.5 \B_{i}
	& \hspace{.5cm}\B_{i+1} &:= 4 \D_{i}\\
\C_1 & := \startWall
	& \D_1		&:= 34 \startWall 
	& \C_2 		&:= 238 \startWall
	& \C_{i+1} 	&:= 7.5 \D_{i}
	& \D_{i+1} 	&:= 4 \B_i,\\
\end{array}
\end{equation*}
which results in the starting intervals given in \autoref{fig:intervalStart}.
The local maxima at $t_1$ and $t_4$ then have \ratio exactly $\nf{17}{9}$. The interval between $t_2$ and $t_3$ is set up equivalent to the one between $t_3$ and $t_6$ in \autoref{fig:recursiveInterlacing}, which means the interlacing construction can be applied to all intervals beyond.
Note that all barriers scale with \mbox{$s$.}
An example of this construction for $\startWall = 1$ is given in \autoref{fig:exampleBarrierSystem}.
\begin{figure}[ht]
	\centering
	\includegraphics[width=.8\textwidth]{figures/StartIntervals2}
	\caption{Illustration of time intervals at the start. Due to their growth, the sizes of the intervals are not true to scale.}
	\label{fig:intervalStart}
\end{figure}
\begin{figure}[ht]
	\centering
	\includegraphics[width=.8\textwidth]{figures/constructionSangSub}
	\caption{Example for the final \crews for $\startWall = 1$, also not true to scale.}
	\label{fig:exampleBarrierSystem}
\end{figure}
\begin{theorem}
The fire can be contained in the upper half-plane with speed $v = \frac{17}{9} =  1.\overline{8}$
\end{theorem}

